Threat Repair with Optimization Modulo Theories

We propose a model-based procedure for automatically preventing security threats using formal models. We encode system models and potential threats as satisfiability modulo theory (SMT) formulas. This model allows us to ask security questions as satisfiability queries. We formulate threat prevention as an optimization problem over the same formulas. The outcome of our threat prevention procedure is a suggestion of model attribute repair that eliminates threats. Whenever threat prevention fails, we automatically explain why the threat happens. We implement our approach using the state-of-the-art Z3 SMT solver and interface it with the threat analysis tool THREATGET. We demonstrate the value of our procedure in two case studies from automotive and smart home domains, including an industrial-strength example.

==> Illustrating/illustrating.tex <==
% \documentclass[multi=tikzpicture]{standalone}
% \input{preamble/packages}
\newcommand{\Wire}{\textcolor{black!50}{\shortstack{Wire\\Connector}}}
\newcommand{\Wireless}{\textcolor{black!50}{\shortstack{Wireless\\Connector}}}
% \begin{document}
    \begin{tikzpicture}[scale=1,transform shape,->,>=latex',auto,node distance=1.5cm,semithick]
        %\small
        \tikzstyle{every state}=[draw=none,rectangle,text=black]
        \node[state] (cloud) {\shortstack{\includegraphics[height=1cm]{Illustrating/cloud-computing.pdf}\\Cloud}};
        \node[state, right= of cloud] (fog) {\shortstack{\includegraphics[height=1cm]{Illustrating/cloud-fog.pdf}\\Fog Node}};
        \node[state, right= of fog] (gateway) {\shortstack{\includegraphics[height=1cm]{IoT/iot-field-gateway.pdf}\\IoT Field\\Gateway}};
        \node[state, right= of gateway] (monitoring) {\shortstack{\includegraphics[height=1cm]{Illustrating/monitoring-svgrepo-com.pdf}\\Intelligent\\Monitoring}};
        \path ($(cloud.east)+(0,0.2)$) edge node {\Wire} ($(fog.west)+(0,0.2)$)
              ($(fog.west)+(0,-0.2)$) edge node {\Wire} ($(cloud.east)+(0,-0.2)$)
              ($(fog.east)+(0,0.2)$) edge node {\Wire} ($(gateway.west)+(0,0.2)$)
              ($(gateway.west)+(0,-0.2)$) edge node {\Wire} ($(fog.east)+(0,-0.2)$)
              ($(gateway.east)+(0,0.2)$) edge node (fw-ws) {\Wireless} ($(monitoring.west)+(0,0.2)$)
              ($(monitoring.west)+(0,-0.2)$) edge node (ws-fw) {\Wireless} ($(gateway.east)+(0,-0.2)$);
    \end{tikzpicture}
% \end{document}

==> content/abstract.tex <==
Measures for preventing threats play an important role in managing risks for securing 
systems. Identifying the minimal effective set of preventive measures is a challenging task that typically requires expert knowledge of security engineers.

We propose a model-based procedure for automatically analyzing and preventing security threats using formal models. We encode architectural system models and %conditions describing 
potential threats as satisfiability modulo theory (SMT) formulas. This model allows us to ask security questions as satisfiability queries. 

We formulate threat prevention as an optimization problem over the same formulas. The outcome of our threat prevention procedure is 
a suggestion of model attribute repair that eliminates threats. Whenever threat prevention fails, 
we automatically explain why the threat happens. We implement our approach using the state-of-the-art Z3 SMT solver and 
interface it with the THREATGET tool for threat modeling and analysis. 
We demonstrate the value of our procedure in three case studies 
from automotive and smart home domains, including an industrial-strength example.

==> content/iot_model.tex <==
\section{Smart Home IoT Model - SMT Encoding}
\label{sec:iotmodel}

\begin{lstlisting}
(declare-datatypes ((AssetType 0)) (((|Confidentiality Asset|) (|Cryptographic Asset|) (PII))))
(declare-datatypes ((StateType 0)) (((Actuator) (|Accelerator Pedal|) (Airbags) (Brakes) (|Electric Actuator|) (Engine) (|Hydraulic Actuator|) (|Pneumatic Actuator|) (Steering) (Antenna) (|Wireless Antenna|) (Application) (|Local Application|) (Backend) (|Third Party Server|) (|Update Server|) (Cloud) (|Database Server|) (|File Server|) (Host) (|Identity Server|) (|IoT Cloud Gateway|) (|Web Server|) (|Communication Element|) (Telematics) (|Wired Bus Communication Element|) (|Wired Communication Element|) (|Wireless Bus Communication Element|) (|Wireless Communication Element|) (|Data Store|) (Cache) (|Cloud HSM|) (|Cloud Storage|) (Database) (|Data Warehouse|) (|Relational Database|) (Device) (|IoT Device|) (|Mobile Client|) (|Smart Device|) (|User Laptop|) (|User Phone|) (|Electronic Control Unit|) (|Communication ECU|) (|High-Performance ECU|) (Immobilizer) (Infotainment) (|Low Performance ECU|) (Microcontroller) (TPMS) (|External Interaction|) (|Central ITS Station|) (|External devices|) (Human) (Vehicle) (|Field Device|) (|Access Point|) (|Field Firewall|) (|IoT Field Gateway|) (Router) (Switch) (Firewall) (Gateway) (|Generic External Interactor|) (Browser) (Interface) (CD) (|GPS Interface|) (|Human Machine Interface|) (|Linkage Interface|) (OBD) (|SD Card|) (USB) (|Wired Interface|) (|Wireless Interface|) (|Key Fob|) (Memory) (|Cloud Data|) (|OnBoard Data|) (Meters) (Battery) (Fuel) (Oil) (Speed) (Temperature) (|Tire Pressure Meter|) (|Network Device|) (Sensor) (|Image Sensor|) (|Contact Sensor|) (|Distance Sensor|) (|Lidar sensor|) (|Non Contact Sensor|) (|Radar Sensor|) (|Ultrasonic Sensor|) (Server) (Service) (ML) (|Mobile App Backend|) (|Web API|) (|Web Application|) (Software) (Applications) (Firmware) (|Smartphone App|) (V2X) (Boundary) (|Car Boundary|) (|Logical Boundary|) (|Physical Boundary|) (|Trusted Environment Boundary|) (|Untrusted Environment Boundary|) (|IaaS VM Trust Boundary|) (|IoT Cloud Gateway Zone|) (|IoT Device Zone|) (|IoT Field Gateway Zone|) (|Local User Zone|) (|Machine Trust Boundary|) (|Remote User Zone|) (|Service Trust Boundary|))))
(declare-datatypes ((StateId 0)) (((|2|) (|3|) (|4|) (|6|) (|10|) (|12|) (|46|) (|47|))))
(declare-datatypes ((contains-relation-sort 0)) (((contains-relation-sort (parent StateId) (child StateId)))))
(declare-datatypes ((AssetId 0)) (((|30|) (|41|))))
(declare-datatypes ((asset-state-relation-sort 0)) (((asset-state-relation-sort (asset AssetId) (state StateId)))))
(declare-datatypes ((AttributeValue 0)) (((missing) (no) (yes) (undefined) (local) (remote) (SQL) (REST) (strong) (Moderate) (Major) (Severe) (Negligible) (No) (Yes) (|Safety oriented|) (|Security oriented|) (low) (high) (deterministic) (Acknowledgment) (retransmission) (encrypted) (|Multi media Data|) (|Control Data|) (|Critical Data|) (|Sensor Data|) (|Configuration Data|) (|Personal Data|) (|ODR Data|) (|Payment account Data|) (|Location Data|) (|salted and hashed|) (None) (|very high|) (medium) (RSA) (DES) (TDES) (SHAone) (MDfive) (incremental) (full) (differential) (checksum) (|Error correction|) (|secure hash|) (Default) (deactivated) (activated) (weak) (|1|) (|2|) (|3|) (|4|) (|5|) (|6|) (|7|) (|8|) (|9|) (|10|) (short) (long) (C) (C++) (Java) (Python) (|closed source (company internal)|) (|open source|) (|third party|) (|On Premise|) (|Off Premise|) (Cloud) (Mobile) (|0|) (|20|) (|40|) (|60|) (|80|) (|100|) (F) (DRAM) (SRAM) (ROM) (NVRAM) (Magnetic) (Optical) (E) (Wireless) (Wired) (Windows) (Linux) (Autosar) (Serious) (Restricted) (User) (Admin) (|own premise|) (multiple) (CAN) (HTTP) (UDP) (HTTPS) (TCP) (|Local Area Wired Network|) (|Local Area Wireless Network|) (|Wide Area Wireless Network|) (double) (triple) (timed) (admin) (user) (manager) (operator) (|on demand|) (continuous) (periodical) (fixed) (executable) (Removeable) (Kmh) (Pa) (mph) (%) (RPM) (software) (firmware) (graphical) (|command line|) (USB) (Ethernet) (FireWire) (GPID) (LIN) (I2C) (SPI) (MOST) (|A��B|) (D2B) (Byteflight) (Flexray) (4G) (5G) (LTE) (GPS) (WiFi) (Bluetooth) (NFC))))
(declare-datatypes ((Attribute 0)) (((|Access Control|) (|Activity Logging|) (Administration) (|Allows User Input|) (|Anomaly Detection|) (|API Type|) (|Approved License|) (Auditing) (Authentication) (Authorization) (Availability) (Bandwidth) (|Certificate Checks|) (|Coding guideline|) (|Communication Latency|) (|Communication Reliability|) (Confidentiality) (Content) (|Counterfeit Detection|) (|Credential Asset|) (Criticality) (|Cryptographic Algorithms|) (|Cryptographic Hardware|) (|Data Backup|) (|Data safety integrity|) (|Data security integrity|) (|Data Store|) (|DDoS Mitigation|) (|Device Fingerprint|) (|Digital Signature|) (Encrypted) (Encryption) (|Encryption Method|) (|Encryption Time|) (|Error Rate|) (Feedback) (|Financial Asset|) (Firmware) (|Input Sanitization|) (|Input Validation|) (Integrity) (|Key Length|) (|Key Revocation|) (Language) (License) (Location) (|Malware Protection|) (Managed) (|Maximum Value|) (|Memory Type|) (|Minimum Value|) (|Network Technology|) (|Operating system|) (|Operational Criticality|) (Permissions) (|Physical Location|) (|Power consumption|) (|Privacy Asset|) (|Processing Time|) (|Protected Execution Environment|) (Protocols) (|Protocol version|) (|PtwoP Capability|) (Range) (Redundancy) (|Reset capabilities|) (Roles) (|Secure Boot|) (|Secure Session Handling|) (|Secure Storage|) (|Secure Update|) (|Sensor measurement type|) (|Shared resources|) (Software) (|Software APIs|) (|Standard Password|) (Storage) (|Tamper Protection|) (|Token Signing|) (|Token Validation|) (Troughput) (Unit) (|Update capabilities|) (Updates) (|URL Blacklisting|) (|User File Upload|) (|User Interfaces|) (|User Management|) (|Wired interface|) (|Wireless Communication Technologie|) (|Wireless Interface|))))
(declare-datatypes ((TransitionType 0)) (((|Communication Flow|) (|Wired Flow|) (|Wireless Flow|) (|Data Flow|) (Request) (Response) (|Internet Connection|) (|Wire Connector|) (|Wireless Connector|))))
(declare-datatypes ((ConnectorId 0)) (((|1|) (|2|) (|10|) (|11|) (|13|) (|14|) (|33|) (|34|) (|36|) (|39|))))
(declare-datatypes ((asset-trans-relation-sort 0)) (((asset-trans-relation-sort (asset AssetId) (trans ConnectorId)))))
(declare-fun is-boundary (StateId) Bool)
(declare-fun state-type (StateId) StateType)
(declare-fun state-attr (StateId Attribute) AttributeValue)
(declare-fun asset-state-relation () (Array asset-state-relation-sort Bool))
(declare-fun contains-relation () (Array contains-relation-sort Bool))
(declare-fun transition-type (ConnectorId) TransitionType)
(declare-fun target (ConnectorId) StateId)
(declare-fun source (ConnectorId) StateId)
(declare-fun trans-attr (ConnectorId Attribute) AttributeValue)
(declare-fun asset-trans-relation () (Array asset-trans-relation-sort Bool))
(declare-fun asset-type (AssetId) AssetType)
(declare-fun asset-attr (AssetId Attribute) AttributeValue)
(assert (= (is-boundary |2|) false))
(assert (= (state-type |2|) Sensor))
(assert (or (= (state-attr |2| Authentication) undefined)
    (= (state-attr |2| Authentication) strong)
    (= (state-attr |2| Authentication) Yes)
    (= (state-attr |2| Authentication) No)
    (= (state-attr |2| Authentication) undefined)
    (= (state-attr |2| Authentication) strong)
    (= (state-attr |2| Authentication) Yes)
    (= (state-attr |2| Authentication) No)
    (= (state-attr |2| Authentication) undefined)
    (= (state-attr |2| Authentication) strong)
    (= (state-attr |2| Authentication) Yes)
    (= (state-attr |2| Authentication) No)))
(assert (or (= (state-attr |2| Authorization) undefined)
    (= (state-attr |2| Authorization) strong)
    (= (state-attr |2| Authorization) Yes)
    (= (state-attr |2| Authorization) No)
    (= (state-attr |2| Authorization) undefined)
    (= (state-attr |2| Authorization) strong)
    (= (state-attr |2| Authorization) Yes)
    (= (state-attr |2| Authorization) No)
    (= (state-attr |2| Authorization) undefined)
    (= (state-attr |2| Authorization) strong)
    (= (state-attr |2| Authorization) Yes)
    (= (state-attr |2| Authorization) No)))
(assert (= (state-attr |2| |Access Control|) missing))
(assert (= (state-attr |2| |Activity Logging|) missing))
(assert (= (state-attr |2| Administration) missing))
(assert (= (state-attr |2| |Allows User Input|) missing))
(assert (= (state-attr |2| |Anomaly Detection|) missing))
(assert (= (state-attr |2| |API Type|) missing))
(assert (= (state-attr |2| |Approved License|) missing))
(assert (= (state-attr |2| Auditing) missing))
(assert (= (state-attr |2| Availability) missing))
(assert (= (state-attr |2| Bandwidth) missing))
(assert (= (state-attr |2| |Certificate Checks|) missing))
(assert (= (state-attr |2| |Coding guideline|) missing))
(assert (= (state-attr |2| |Communication Latency|) missing))
(assert (= (state-attr |2| |Communication Reliability|) missing))
(assert (= (state-attr |2| Confidentiality) missing))
(assert (= (state-attr |2| Content) missing))
(assert (= (state-attr |2| |Counterfeit Detection|) missing))
(assert (= (state-attr |2| |Credential Asset|) missing))
(assert (= (state-attr |2| Criticality) missing))
(assert (= (state-attr |2| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |2| |Cryptographic Hardware|) missing))
(assert (= (state-attr |2| |Data Backup|) missing))
(assert (= (state-attr |2| |Data safety integrity|) missing))
(assert (= (state-attr |2| |Data security integrity|) missing))
(assert (= (state-attr |2| |Data Store|) missing))
(assert (= (state-attr |2| |DDoS Mitigation|) missing))
(assert (= (state-attr |2| |Device Fingerprint|) missing))
(assert (= (state-attr |2| |Digital Signature|) missing))
(assert (= (state-attr |2| Encrypted) missing))
(assert (= (state-attr |2| Encryption) missing))
(assert (= (state-attr |2| |Encryption Method|) missing))
(assert (= (state-attr |2| |Encryption Time|) missing))
(assert (= (state-attr |2| |Error Rate|) missing))
(assert (= (state-attr |2| Feedback) missing))
(assert (= (state-attr |2| |Financial Asset|) missing))
(assert (= (state-attr |2| Firmware) missing))
(assert (= (state-attr |2| |Input Sanitization|) missing))
(assert (= (state-attr |2| |Input Validation|) missing))
(assert (= (state-attr |2| Integrity) missing))
(assert (= (state-attr |2| |Key Length|) missing))
(assert (= (state-attr |2| |Key Revocation|) missing))
(assert (= (state-attr |2| Language) missing))
(assert (= (state-attr |2| License) missing))
(assert (= (state-attr |2| Location) missing))
(assert (= (state-attr |2| |Malware Protection|) missing))
(assert (= (state-attr |2| Managed) missing))
(assert (= (state-attr |2| |Maximum Value|) missing))
(assert (= (state-attr |2| |Memory Type|) missing))
(assert (= (state-attr |2| |Minimum Value|) missing))
(assert (= (state-attr |2| |Network Technology|) missing))
(assert (= (state-attr |2| |Operating system|) missing))
(assert (= (state-attr |2| |Operational Criticality|) missing))
(assert (= (state-attr |2| Permissions) missing))
(assert (= (state-attr |2| |Physical Location|) missing))
(assert (= (state-attr |2| |Power consumption|) missing))
(assert (= (state-attr |2| |Privacy Asset|) missing))
(assert (= (state-attr |2| |Processing Time|) missing))
(assert (= (state-attr |2| |Protected Execution Environment|) missing))
(assert (= (state-attr |2| |Protocol version|) missing))
(assert (= (state-attr |2| Protocols) missing))
(assert (= (state-attr |2| |PtwoP Capability|) missing))
(assert (= (state-attr |2| Range) missing))
(assert (= (state-attr |2| Redundancy) missing))
(assert (= (state-attr |2| |Reset capabilities|) missing))
(assert (= (state-attr |2| Roles) missing))
(assert (= (state-attr |2| |Secure Boot|) missing))
(assert (= (state-attr |2| |Secure Session Handling|) missing))
(assert (= (state-attr |2| |Secure Storage|) missing))
(assert (= (state-attr |2| |Secure Update|) missing))
(assert (= (state-attr |2| |Sensor measurement type|) missing))
(assert (= (state-attr |2| |Shared resources|) missing))
(assert (= (state-attr |2| Software) missing))
(assert (= (state-attr |2| |Software APIs|) missing))
(assert (= (state-attr |2| |Standard Password|) missing))
(assert (= (state-attr |2| Storage) missing))
(assert (= (state-attr |2| |Tamper Protection|) missing))
(assert (= (state-attr |2| |Token Signing|) missing))
(assert (= (state-attr |2| |Token Validation|) missing))
(assert (= (state-attr |2| Troughput) missing))
(assert (= (state-attr |2| Unit) missing))
(assert (= (state-attr |2| |Update capabilities|) missing))
(assert (= (state-attr |2| Updates) missing))
(assert (= (state-attr |2| |URL Blacklisting|) missing))
(assert (= (state-attr |2| |User File Upload|) missing))
(assert (= (state-attr |2| |User Interfaces|) missing))
(assert (= (state-attr |2| |User Management|) missing))
(assert (= (state-attr |2| |Wired interface|) missing))
(assert (= (state-attr |2| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |2| |Wireless Interface|) missing))
(assert (= (is-boundary |3|) false))
(assert (= (state-type |3|) |User Phone|))
(assert (or (= (state-attr |3| |Allows User Input|) undefined)
    (= (state-attr |3| |Allows User Input|) Yes)
    (= (state-attr |3| |Allows User Input|) No)
    (= (state-attr |3| |Allows User Input|) undefined)
    (= (state-attr |3| |Allows User Input|) Yes)
    (= (state-attr |3| |Allows User Input|) No)
    (= (state-attr |3| |Allows User Input|) undefined)
    (= (state-attr |3| |Allows User Input|) Yes)
    (= (state-attr |3| |Allows User Input|) No)))
(assert (or (= (state-attr |3| |Approved License|) undefined)
    (= (state-attr |3| |Approved License|) Yes)
    (= (state-attr |3| |Approved License|) No)
    (= (state-attr |3| |Approved License|) undefined)
    (= (state-attr |3| |Approved License|) Yes)
    (= (state-attr |3| |Approved License|) No)
    (= (state-attr |3| |Approved License|) undefined)
    (= (state-attr |3| |Approved License|) Yes)
    (= (state-attr |3| |Approved License|) No)))
(assert (or (= (state-attr |3| Authentication) undefined)
    (= (state-attr |3| Authentication) strong)
    (= (state-attr |3| Authentication) Yes)
    (= (state-attr |3| Authentication) No)
    (= (state-attr |3| Authentication) undefined)
    (= (state-attr |3| Authentication) strong)
    (= (state-attr |3| Authentication) Yes)
    (= (state-attr |3| Authentication) No)
    (= (state-attr |3| Authentication) undefined)
    (= (state-attr |3| Authentication) strong)
    (= (state-attr |3| Authentication) Yes)
    (= (state-attr |3| Authentication) No)))
(assert (or (= (state-attr |3| Authorization) undefined)
    (= (state-attr |3| Authorization) strong)
    (= (state-attr |3| Authorization) Yes)
    (= (state-attr |3| Authorization) No)
    (= (state-attr |3| Authorization) undefined)
    (= (state-attr |3| Authorization) strong)
    (= (state-attr |3| Authorization) Yes)
    (= (state-attr |3| Authorization) No)
    (= (state-attr |3| Authorization) undefined)
    (= (state-attr |3| Authorization) strong)
    (= (state-attr |3| Authorization) Yes)
    (= (state-attr |3| Authorization) No)))
(assert (or (= (state-attr |3| |Certificate Checks|) undefined)
    (= (state-attr |3| |Certificate Checks|) Yes)
    (= (state-attr |3| |Certificate Checks|) No)
    (= (state-attr |3| |Certificate Checks|) undefined)
    (= (state-attr |3| |Certificate Checks|) Yes)
    (= (state-attr |3| |Certificate Checks|) No)
    (= (state-attr |3| |Certificate Checks|) undefined)
    (= (state-attr |3| |Certificate Checks|) Yes)
    (= (state-attr |3| |Certificate Checks|) No)))
(assert (or (= (state-attr |3| |Counterfeit Detection|) undefined)
    (= (state-attr |3| |Counterfeit Detection|) No)
    (= (state-attr |3| |Counterfeit Detection|) Yes)
    (= (state-attr |3| |Counterfeit Detection|) undefined)
    (= (state-attr |3| |Counterfeit Detection|) No)
    (= (state-attr |3| |Counterfeit Detection|) Yes)
    (= (state-attr |3| |Counterfeit Detection|) undefined)
    (= (state-attr |3| |Counterfeit Detection|) No)
    (= (state-attr |3| |Counterfeit Detection|) Yes)))
(assert (or (= (state-attr |3| |Cryptographic Hardware|) undefined)
    (= (state-attr |3| |Cryptographic Hardware|) Yes)
    (= (state-attr |3| |Cryptographic Hardware|) No)
    (= (state-attr |3| |Cryptographic Hardware|) undefined)
    (= (state-attr |3| |Cryptographic Hardware|) Yes)
    (= (state-attr |3| |Cryptographic Hardware|) No)
    (= (state-attr |3| |Cryptographic Hardware|) undefined)
    (= (state-attr |3| |Cryptographic Hardware|) Yes)
    (= (state-attr |3| |Cryptographic Hardware|) No)))
(assert (or (= (state-attr |3| Encrypted) undefined)
    (= (state-attr |3| Encrypted) Yes)
    (= (state-attr |3| Encrypted) No)
    (= (state-attr |3| Encrypted) strong)
    (= (state-attr |3| Encrypted) undefined)
    (= (state-attr |3| Encrypted) Yes)
    (= (state-attr |3| Encrypted) No)
    (= (state-attr |3| Encrypted) strong)
    (= (state-attr |3| Encrypted) undefined)
    (= (state-attr |3| Encrypted) Yes)
    (= (state-attr |3| Encrypted) No)
    (= (state-attr |3| Encrypted) strong)))
(assert (or (= (state-attr |3| |Encryption Method|) undefined)
    (= (state-attr |3| |Encryption Method|) strong)
    (= (state-attr |3| |Encryption Method|) weak)
    (= (state-attr |3| |Encryption Method|) undefined)
    (= (state-attr |3| |Encryption Method|) strong)
    (= (state-attr |3| |Encryption Method|) weak)
    (= (state-attr |3| |Encryption Method|) undefined)
    (= (state-attr |3| |Encryption Method|) strong)
    (= (state-attr |3| |Encryption Method|) weak)))
(assert (or (= (state-attr |3| |Financial Asset|) undefined)
    (= (state-attr |3| |Financial Asset|) Yes)
    (= (state-attr |3| |Financial Asset|) No)
    (= (state-attr |3| |Financial Asset|) undefined)
    (= (state-attr |3| |Financial Asset|) Yes)
    (= (state-attr |3| |Financial Asset|) No)
    (= (state-attr |3| |Financial Asset|) undefined)
    (= (state-attr |3| |Financial Asset|) Yes)
    (= (state-attr |3| |Financial Asset|) No)))
(assert (or (= (state-attr |3| Location) undefined)
    (= (state-attr |3| Location) |On Premise|)
    (= (state-attr |3| Location) |Off Premise|)
    (= (state-attr |3| Location) Cloud)
    (= (state-attr |3| Location) Mobile)
    (= (state-attr |3| Location) undefined)
    (= (state-attr |3| Location) |On Premise|)
    (= (state-attr |3| Location) |Off Premise|)
    (= (state-attr |3| Location) Cloud)
    (= (state-attr |3| Location) Mobile)
    (= (state-attr |3| Location) undefined)
    (= (state-attr |3| Location) |On Premise|)
    (= (state-attr |3| Location) |Off Premise|)
    (= (state-attr |3| Location) Cloud)
    (= (state-attr |3| Location) Mobile)))
(assert (or (= (state-attr |3| |Malware Protection|) undefined)
    (= (state-attr |3| |Malware Protection|) Yes)
    (= (state-attr |3| |Malware Protection|) No)
    (= (state-attr |3| |Malware Protection|) undefined)
    (= (state-attr |3| |Malware Protection|) Yes)
    (= (state-attr |3| |Malware Protection|) No)
    (= (state-attr |3| |Malware Protection|) undefined)
    (= (state-attr |3| |Malware Protection|) Yes)
    (= (state-attr |3| |Malware Protection|) No)))
(assert (or (= (state-attr |3| Managed) undefined)
    (= (state-attr |3| Managed) No)
    (= (state-attr |3| Managed) Yes)
    (= (state-attr |3| Managed) undefined)
    (= (state-attr |3| Managed) No)
    (= (state-attr |3| Managed) Yes)
    (= (state-attr |3| Managed) undefined)
    (= (state-attr |3| Managed) No)
    (= (state-attr |3| Managed) Yes)))
(assert (or (= (state-attr |3| |Privacy Asset|) undefined)
    (= (state-attr |3| |Privacy Asset|) Yes)
    (= (state-attr |3| |Privacy Asset|) No)
    (= (state-attr |3| |Privacy Asset|) multiple)
    (= (state-attr |3| |Privacy Asset|) undefined)
    (= (state-attr |3| |Privacy Asset|) Yes)
    (= (state-attr |3| |Privacy Asset|) No)
    (= (state-attr |3| |Privacy Asset|) multiple)
    (= (state-attr |3| |Privacy Asset|) undefined)
    (= (state-attr |3| |Privacy Asset|) Yes)
    (= (state-attr |3| |Privacy Asset|) No)
    (= (state-attr |3| |Privacy Asset|) multiple)))
(assert (or (= (state-attr |3| |Protected Execution Environment|) undefined)
    (= (state-attr |3| |Protected Execution Environment|) Yes)
    (= (state-attr |3| |Protected Execution Environment|) No)
    (= (state-attr |3| |Protected Execution Environment|) undefined)
    (= (state-attr |3| |Protected Execution Environment|) Yes)
    (= (state-attr |3| |Protected Execution Environment|) No)
    (= (state-attr |3| |Protected Execution Environment|) undefined)
    (= (state-attr |3| |Protected Execution Environment|) Yes)
    (= (state-attr |3| |Protected Execution Environment|) No)))
(assert (or (= (state-attr |3| |PtwoP Capability|) undefined)
    (= (state-attr |3| |PtwoP Capability|) Yes)
    (= (state-attr |3| |PtwoP Capability|) No)
    (= (state-attr |3| |PtwoP Capability|) undefined)
    (= (state-attr |3| |PtwoP Capability|) Yes)
    (= (state-attr |3| |PtwoP Capability|) No)
    (= (state-attr |3| |PtwoP Capability|) undefined)
    (= (state-attr |3| |PtwoP Capability|) Yes)
    (= (state-attr |3| |PtwoP Capability|) No)))
(assert (or (= (state-attr |3| |Secure Session Handling|) undefined)
    (= (state-attr |3| |Secure Session Handling|) Yes)
    (= (state-attr |3| |Secure Session Handling|) No)
    (= (state-attr |3| |Secure Session Handling|) undefined)
    (= (state-attr |3| |Secure Session Handling|) Yes)
    (= (state-attr |3| |Secure Session Handling|) No)
    (= (state-attr |3| |Secure Session Handling|) undefined)
    (= (state-attr |3| |Secure Session Handling|) Yes)
    (= (state-attr |3| |Secure Session Handling|) No)))
(assert (or (= (state-attr |3| |Standard Password|) undefined)
    (= (state-attr |3| |Standard Password|) Yes)
    (= (state-attr |3| |Standard Password|) No)
    (= (state-attr |3| |Standard Password|) undefined)
    (= (state-attr |3| |Standard Password|) Yes)
    (= (state-attr |3| |Standard Password|) No)
    (= (state-attr |3| |Standard Password|) undefined)
    (= (state-attr |3| |Standard Password|) Yes)
    (= (state-attr |3| |Standard Password|) No)))
(assert (or (= (state-attr |3| Storage) undefined)
    (= (state-attr |3| Storage) Removeable)
    (= (state-attr |3| Storage) undefined)
    (= (state-attr |3| Storage) Removeable)
    (= (state-attr |3| Storage) undefined)
    (= (state-attr |3| Storage) Removeable)))
(assert (or (= (state-attr |3| |Tamper Protection|) Yes)
    (= (state-attr |3| |Tamper Protection|) No)
    (= (state-attr |3| |Tamper Protection|) undefined)))
(assert (or (= (state-attr |3| |Token Signing|) undefined)
    (= (state-attr |3| |Token Signing|) Yes)
    (= (state-attr |3| |Token Signing|) No)
    (= (state-attr |3| |Token Signing|) undefined)
    (= (state-attr |3| |Token Signing|) Yes)
    (= (state-attr |3| |Token Signing|) No)
    (= (state-attr |3| |Token Signing|) undefined)
    (= (state-attr |3| |Token Signing|) Yes)
    (= (state-attr |3| |Token Signing|) No)))
(assert (or (= (state-attr |3| |URL Blacklisting|) undefined)
    (= (state-attr |3| |URL Blacklisting|) Yes)
    (= (state-attr |3| |URL Blacklisting|) No)
    (= (state-attr |3| |URL Blacklisting|) undefined)
    (= (state-attr |3| |URL Blacklisting|) Yes)
    (= (state-attr |3| |URL Blacklisting|) No)
    (= (state-attr |3| |URL Blacklisting|) undefined)
    (= (state-attr |3| |URL Blacklisting|) Yes)
    (= (state-attr |3| |URL Blacklisting|) No)))
(assert (= (state-attr |3| |Access Control|) missing))
(assert (= (state-attr |3| |Activity Logging|) missing))
(assert (= (state-attr |3| Administration) missing))
(assert (= (state-attr |3| |Anomaly Detection|) missing))
(assert (= (state-attr |3| |API Type|) missing))
(assert (= (state-attr |3| Auditing) missing))
(assert (= (state-attr |3| Availability) missing))
(assert (= (state-attr |3| Bandwidth) missing))
(assert (= (state-attr |3| |Coding guideline|) missing))
(assert (= (state-attr |3| |Communication Latency|) missing))
(assert (= (state-attr |3| |Communication Reliability|) missing))
(assert (= (state-attr |3| Confidentiality) missing))
(assert (= (state-attr |3| Content) missing))
(assert (= (state-attr |3| |Credential Asset|) missing))
(assert (= (state-attr |3| Criticality) missing))
(assert (= (state-attr |3| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |3| |Data Backup|) missing))
(assert (= (state-attr |3| |Data safety integrity|) missing))
(assert (= (state-attr |3| |Data security integrity|) missing))
(assert (= (state-attr |3| |Data Store|) missing))
(assert (= (state-attr |3| |DDoS Mitigation|) missing))
(assert (= (state-attr |3| |Device Fingerprint|) missing))
(assert (= (state-attr |3| |Digital Signature|) missing))
(assert (= (state-attr |3| Encryption) missing))
(assert (= (state-attr |3| |Encryption Time|) missing))
(assert (= (state-attr |3| |Error Rate|) missing))
(assert (= (state-attr |3| Feedback) missing))
(assert (= (state-attr |3| Firmware) missing))
(assert (= (state-attr |3| |Input Sanitization|) missing))
(assert (= (state-attr |3| |Input Validation|) missing))
(assert (= (state-attr |3| Integrity) missing))
(assert (= (state-attr |3| |Key Length|) missing))
(assert (= (state-attr |3| |Key Revocation|) missing))
(assert (= (state-attr |3| Language) missing))
(assert (= (state-attr |3| License) missing))
(assert (= (state-attr |3| |Maximum Value|) missing))
(assert (= (state-attr |3| |Memory Type|) missing))
(assert (= (state-attr |3| |Minimum Value|) missing))
(assert (= (state-attr |3| |Network Technology|) missing))
(assert (= (state-attr |3| |Operating system|) missing))
(assert (= (state-attr |3| |Operational Criticality|) missing))
(assert (= (state-attr |3| Permissions) missing))
(assert (= (state-attr |3| |Physical Location|) missing))
(assert (= (state-attr |3| |Power consumption|) missing))
(assert (= (state-attr |3| |Processing Time|) missing))
(assert (= (state-attr |3| |Protocol version|) missing))
(assert (= (state-attr |3| Protocols) missing))
(assert (= (state-attr |3| Range) missing))
(assert (= (state-attr |3| Redundancy) missing))
(assert (= (state-attr |3| |Reset capabilities|) missing))
(assert (= (state-attr |3| Roles) missing))
(assert (= (state-attr |3| |Secure Boot|) missing))
(assert (= (state-attr |3| |Secure Storage|) missing))
(assert (= (state-attr |3| |Secure Update|) missing))
(assert (= (state-attr |3| |Sensor measurement type|) missing))
(assert (= (state-attr |3| |Shared resources|) missing))
(assert (= (state-attr |3| Software) missing))
(assert (= (state-attr |3| |Software APIs|) missing))
(assert (= (state-attr |3| |Token Validation|) missing))
(assert (= (state-attr |3| Troughput) missing))
(assert (= (state-attr |3| Unit) missing))
(assert (= (state-attr |3| |Update capabilities|) missing))
(assert (= (state-attr |3| Updates) missing))
(assert (= (state-attr |3| |User File Upload|) missing))
(assert (= (state-attr |3| |User Interfaces|) missing))
(assert (= (state-attr |3| |User Management|) missing))
(assert (= (state-attr |3| |Wired interface|) missing))
(assert (= (state-attr |3| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |3| |Wireless Interface|) missing))
(assert (= (is-boundary |4|) false))
(assert (= (state-type |4|) Sensor))
(assert (or (= (state-attr |4| Authentication) undefined)
    (= (state-attr |4| Authentication) strong)
    (= (state-attr |4| Authentication) Yes)
    (= (state-attr |4| Authentication) No)
    (= (state-attr |4| Authentication) undefined)
    (= (state-attr |4| Authentication) strong)
    (= (state-attr |4| Authentication) Yes)
    (= (state-attr |4| Authentication) No)
    (= (state-attr |4| Authentication) undefined)
    (= (state-attr |4| Authentication) strong)
    (= (state-attr |4| Authentication) Yes)
    (= (state-attr |4| Authentication) No)))
(assert (or (= (state-attr |4| Authorization) undefined)
    (= (state-attr |4| Authorization) strong)
    (= (state-attr |4| Authorization) Yes)
    (= (state-attr |4| Authorization) No)
    (= (state-attr |4| Authorization) undefined)
    (= (state-attr |4| Authorization) strong)
    (= (state-attr |4| Authorization) Yes)
    (= (state-attr |4| Authorization) No)
    (= (state-attr |4| Authorization) undefined)
    (= (state-attr |4| Authorization) strong)
    (= (state-attr |4| Authorization) Yes)
    (= (state-attr |4| Authorization) No)))
(assert (= (state-attr |4| |Access Control|) missing))
(assert (= (state-attr |4| |Activity Logging|) missing))
(assert (= (state-attr |4| Administration) missing))
(assert (= (state-attr |4| |Allows User Input|) missing))
(assert (= (state-attr |4| |Anomaly Detection|) missing))
(assert (= (state-attr |4| |API Type|) missing))
(assert (= (state-attr |4| |Approved License|) missing))
(assert (= (state-attr |4| Auditing) missing))
(assert (= (state-attr |4| Availability) missing))
(assert (= (state-attr |4| Bandwidth) missing))
(assert (= (state-attr |4| |Certificate Checks|) missing))
(assert (= (state-attr |4| |Coding guideline|) missing))
(assert (= (state-attr |4| |Communication Latency|) missing))
(assert (= (state-attr |4| |Communication Reliability|) missing))
(assert (= (state-attr |4| Confidentiality) missing))
(assert (= (state-attr |4| Content) missing))
(assert (= (state-attr |4| |Counterfeit Detection|) missing))
(assert (= (state-attr |4| |Credential Asset|) missing))
(assert (= (state-attr |4| Criticality) missing))
(assert (= (state-attr |4| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |4| |Cryptographic Hardware|) missing))
(assert (= (state-attr |4| |Data Backup|) missing))
(assert (= (state-attr |4| |Data safety integrity|) missing))
(assert (= (state-attr |4| |Data security integrity|) missing))
(assert (= (state-attr |4| |Data Store|) missing))
(assert (= (state-attr |4| |DDoS Mitigation|) missing))
(assert (= (state-attr |4| |Device Fingerprint|) missing))
(assert (= (state-attr |4| |Digital Signature|) missing))
(assert (= (state-attr |4| Encrypted) missing))
(assert (= (state-attr |4| Encryption) missing))
(assert (= (state-attr |4| |Encryption Method|) missing))
(assert (= (state-attr |4| |Encryption Time|) missing))
(assert (= (state-attr |4| |Error Rate|) missing))
(assert (= (state-attr |4| Feedback) missing))
(assert (= (state-attr |4| |Financial Asset|) missing))
(assert (= (state-attr |4| Firmware) missing))
(assert (= (state-attr |4| |Input Sanitization|) missing))
(assert (= (state-attr |4| |Input Validation|) missing))
(assert (= (state-attr |4| Integrity) missing))
(assert (= (state-attr |4| |Key Length|) missing))
(assert (= (state-attr |4| |Key Revocation|) missing))
(assert (= (state-attr |4| Language) missing))
(assert (= (state-attr |4| License) missing))
(assert (= (state-attr |4| Location) missing))
(assert (= (state-attr |4| |Malware Protection|) missing))
(assert (= (state-attr |4| Managed) missing))
(assert (= (state-attr |4| |Maximum Value|) missing))
(assert (= (state-attr |4| |Memory Type|) missing))
(assert (= (state-attr |4| |Minimum Value|) missing))
(assert (= (state-attr |4| |Network Technology|) missing))
(assert (= (state-attr |4| |Operating system|) missing))
(assert (= (state-attr |4| |Operational Criticality|) missing))
(assert (= (state-attr |4| Permissions) missing))
(assert (= (state-attr |4| |Physical Location|) missing))
(assert (= (state-attr |4| |Power consumption|) missing))
(assert (= (state-attr |4| |Privacy Asset|) missing))
(assert (= (state-attr |4| |Processing Time|) missing))
(assert (= (state-attr |4| |Protected Execution Environment|) missing))
(assert (= (state-attr |4| |Protocol version|) missing))
(assert (= (state-attr |4| Protocols) missing))
(assert (= (state-attr |4| |PtwoP Capability|) missing))
(assert (= (state-attr |4| Range) missing))
(assert (= (state-attr |4| Redundancy) missing))
(assert (= (state-attr |4| |Reset capabilities|) missing))
(assert (= (state-attr |4| Roles) missing))
(assert (= (state-attr |4| |Secure Boot|) missing))
(assert (= (state-attr |4| |Secure Session Handling|) missing))
(assert (= (state-attr |4| |Secure Storage|) missing))
(assert (= (state-attr |4| |Secure Update|) missing))
(assert (= (state-attr |4| |Sensor measurement type|) missing))
(assert (= (state-attr |4| |Shared resources|) missing))
(assert (= (state-attr |4| Software) missing))
(assert (= (state-attr |4| |Software APIs|) missing))
(assert (= (state-attr |4| |Standard Password|) missing))
(assert (= (state-attr |4| Storage) missing))
(assert (= (state-attr |4| |Tamper Protection|) missing))
(assert (= (state-attr |4| |Token Signing|) missing))
(assert (= (state-attr |4| |Token Validation|) missing))
(assert (= (state-attr |4| Troughput) missing))
(assert (= (state-attr |4| Unit) missing))
(assert (= (state-attr |4| |Update capabilities|) missing))
(assert (= (state-attr |4| Updates) missing))
(assert (= (state-attr |4| |URL Blacklisting|) missing))
(assert (= (state-attr |4| |User File Upload|) missing))
(assert (= (state-attr |4| |User Interfaces|) missing))
(assert (= (state-attr |4| |User Management|) missing))
(assert (= (state-attr |4| |Wired interface|) missing))
(assert (= (state-attr |4| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |4| |Wireless Interface|) missing))
(assert (= (is-boundary |6|) false))
(assert (= (state-type |6|) |IoT Field Gateway|))
(assert (or (= (state-attr |6| |Activity Logging|) undefined)
    (= (state-attr |6| |Activity Logging|) Yes)
    (= (state-attr |6| |Activity Logging|) No)
    (= (state-attr |6| |Activity Logging|) undefined)
    (= (state-attr |6| |Activity Logging|) Yes)
    (= (state-attr |6| |Activity Logging|) No)
    (= (state-attr |6| |Activity Logging|) undefined)
    (= (state-attr |6| |Activity Logging|) Yes)
    (= (state-attr |6| |Activity Logging|) No)))
(assert (or (= (state-attr |6| |Allows User Input|) undefined)
    (= (state-attr |6| |Allows User Input|) Yes)
    (= (state-attr |6| |Allows User Input|) No)
    (= (state-attr |6| |Allows User Input|) undefined)
    (= (state-attr |6| |Allows User Input|) Yes)
    (= (state-attr |6| |Allows User Input|) No)
    (= (state-attr |6| |Allows User Input|) undefined)
    (= (state-attr |6| |Allows User Input|) Yes)
    (= (state-attr |6| |Allows User Input|) No)))
(assert (or (= (state-attr |6| |Anomaly Detection|) undefined)
    (= (state-attr |6| |Anomaly Detection|) Yes)
    (= (state-attr |6| |Anomaly Detection|) No)
    (= (state-attr |6| |Anomaly Detection|) undefined)
    (= (state-attr |6| |Anomaly Detection|) Yes)
    (= (state-attr |6| |Anomaly Detection|) No)
    (= (state-attr |6| |Anomaly Detection|) undefined)
    (= (state-attr |6| |Anomaly Detection|) Yes)
    (= (state-attr |6| |Anomaly Detection|) No)))
(assert (or (= (state-attr |6| Authentication) undefined)
    (= (state-attr |6| Authentication) strong)
    (= (state-attr |6| Authentication) Yes)
    (= (state-attr |6| Authentication) No)
    (= (state-attr |6| Authentication) undefined)
    (= (state-attr |6| Authentication) strong)
    (= (state-attr |6| Authentication) Yes)
    (= (state-attr |6| Authentication) No)
    (= (state-attr |6| Authentication) undefined)
    (= (state-attr |6| Authentication) strong)
    (= (state-attr |6| Authentication) Yes)
    (= (state-attr |6| Authentication) No)))
(assert (or (= (state-attr |6| Authorization) undefined)
    (= (state-attr |6| Authorization) strong)
    (= (state-attr |6| Authorization) Yes)
    (= (state-attr |6| Authorization) No)
    (= (state-attr |6| Authorization) undefined)
    (= (state-attr |6| Authorization) strong)
    (= (state-attr |6| Authorization) Yes)
    (= (state-attr |6| Authorization) No)
    (= (state-attr |6| Authorization) undefined)
    (= (state-attr |6| Authorization) strong)
    (= (state-attr |6| Authorization) Yes)
    (= (state-attr |6| Authorization) No)))
(assert (or (= (state-attr |6| |Credential Asset|) undefined)
    (= (state-attr |6| |Credential Asset|) Yes)
    (= (state-attr |6| |Credential Asset|) No)
    (= (state-attr |6| |Credential Asset|) encrypted)
    (= (state-attr |6| |Credential Asset|) |salted and hashed|)
    (= (state-attr |6| |Credential Asset|) undefined)
    (= (state-attr |6| |Credential Asset|) Yes)
    (= (state-attr |6| |Credential Asset|) No)
    (= (state-attr |6| |Credential Asset|) encrypted)
    (= (state-attr |6| |Credential Asset|) |salted and hashed|)
    (= (state-attr |6| |Credential Asset|) undefined)
    (= (state-attr |6| |Credential Asset|) Yes)
    (= (state-attr |6| |Credential Asset|) No)
    (= (state-attr |6| |Credential Asset|) encrypted)
    (= (state-attr |6| |Credential Asset|) |salted and hashed|)))
(assert (or (= (state-attr |6| |Cryptographic Hardware|) undefined)
    (= (state-attr |6| |Cryptographic Hardware|) Yes)
    (= (state-attr |6| |Cryptographic Hardware|) No)
    (= (state-attr |6| |Cryptographic Hardware|) undefined)
    (= (state-attr |6| |Cryptographic Hardware|) Yes)
    (= (state-attr |6| |Cryptographic Hardware|) No)
    (= (state-attr |6| |Cryptographic Hardware|) undefined)
    (= (state-attr |6| |Cryptographic Hardware|) Yes)
    (= (state-attr |6| |Cryptographic Hardware|) No)))
(assert (or (= (state-attr |6| |Device Fingerprint|) undefined)
    (= (state-attr |6| |Device Fingerprint|) deactivated)
    (= (state-attr |6| |Device Fingerprint|) activated)
    (= (state-attr |6| |Device Fingerprint|) undefined)
    (= (state-attr |6| |Device Fingerprint|) deactivated)
    (= (state-attr |6| |Device Fingerprint|) activated)
    (= (state-attr |6| |Device Fingerprint|) undefined)
    (= (state-attr |6| |Device Fingerprint|) deactivated)
    (= (state-attr |6| |Device Fingerprint|) activated)))
(assert (or (= (state-attr |6| Encrypted) undefined)
    (= (state-attr |6| Encrypted) Yes)
    (= (state-attr |6| Encrypted) No)
    (= (state-attr |6| Encrypted) strong)
    (= (state-attr |6| Encrypted) undefined)
    (= (state-attr |6| Encrypted) Yes)
    (= (state-attr |6| Encrypted) No)
    (= (state-attr |6| Encrypted) strong)
    (= (state-attr |6| Encrypted) undefined)
    (= (state-attr |6| Encrypted) Yes)
    (= (state-attr |6| Encrypted) No)
    (= (state-attr |6| Encrypted) strong)))
(assert (or (= (state-attr |6| |Input Sanitization|) Yes)
    (= (state-attr |6| |Input Sanitization|) No)
    (= (state-attr |6| |Input Sanitization|) undefined)))
(assert (or (= (state-attr |6| |Malware Protection|) undefined)
    (= (state-attr |6| |Malware Protection|) Yes)
    (= (state-attr |6| |Malware Protection|) No)
    (= (state-attr |6| |Malware Protection|) undefined)
    (= (state-attr |6| |Malware Protection|) Yes)
    (= (state-attr |6| |Malware Protection|) No)
    (= (state-attr |6| |Malware Protection|) undefined)
    (= (state-attr |6| |Malware Protection|) Yes)
    (= (state-attr |6| |Malware Protection|) No)))
(assert (or (= (state-attr |6| Managed) undefined)
    (= (state-attr |6| Managed) No)
    (= (state-attr |6| Managed) Yes)
    (= (state-attr |6| Managed) undefined)
    (= (state-attr |6| Managed) No)
    (= (state-attr |6| Managed) Yes)
    (= (state-attr |6| Managed) undefined)
    (= (state-attr |6| Managed) No)
    (= (state-attr |6| Managed) Yes)))
(assert (or (= (state-attr |6| |Protected Execution Environment|) undefined)
    (= (state-attr |6| |Protected Execution Environment|) Yes)
    (= (state-attr |6| |Protected Execution Environment|) No)
    (= (state-attr |6| |Protected Execution Environment|) undefined)
    (= (state-attr |6| |Protected Execution Environment|) Yes)
    (= (state-attr |6| |Protected Execution Environment|) No)
    (= (state-attr |6| |Protected Execution Environment|) undefined)
    (= (state-attr |6| |Protected Execution Environment|) Yes)
    (= (state-attr |6| |Protected Execution Environment|) No)))
(assert (or (= (state-attr |6| |Standard Password|) undefined)
    (= (state-attr |6| |Standard Password|) Yes)
    (= (state-attr |6| |Standard Password|) No)
    (= (state-attr |6| |Standard Password|) undefined)
    (= (state-attr |6| |Standard Password|) Yes)
    (= (state-attr |6| |Standard Password|) No)
    (= (state-attr |6| |Standard Password|) undefined)
    (= (state-attr |6| |Standard Password|) Yes)
    (= (state-attr |6| |Standard Password|) No)))
(assert (or (= (state-attr |6| |Tamper Protection|) Yes)
    (= (state-attr |6| |Tamper Protection|) No)
    (= (state-attr |6| |Tamper Protection|) undefined)))
(assert (or (= (state-attr |6| |Token Validation|) undefined)
    (= (state-attr |6| |Token Validation|) Yes)
    (= (state-attr |6| |Token Validation|) No)
    (= (state-attr |6| |Token Validation|) undefined)
    (= (state-attr |6| |Token Validation|) Yes)
    (= (state-attr |6| |Token Validation|) No)
    (= (state-attr |6| |Token Validation|) undefined)
    (= (state-attr |6| |Token Validation|) Yes)
    (= (state-attr |6| |Token Validation|) No)))
(assert (= (state-attr |6| |Access Control|) missing))
(assert (= (state-attr |6| Administration) missing))
(assert (= (state-attr |6| |API Type|) missing))
(assert (= (state-attr |6| |Approved License|) missing))
(assert (= (state-attr |6| Auditing) missing))
(assert (= (state-attr |6| Availability) missing))
(assert (= (state-attr |6| Bandwidth) missing))
(assert (= (state-attr |6| |Certificate Checks|) missing))
(assert (= (state-attr |6| |Coding guideline|) missing))
(assert (= (state-attr |6| |Communication Latency|) missing))
(assert (= (state-attr |6| |Communication Reliability|) missing))
(assert (= (state-attr |6| Confidentiality) missing))
(assert (= (state-attr |6| Content) missing))
(assert (= (state-attr |6| |Counterfeit Detection|) missing))
(assert (= (state-attr |6| Criticality) missing))
(assert (= (state-attr |6| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |6| |Data Backup|) missing))
(assert (= (state-attr |6| |Data safety integrity|) missing))
(assert (= (state-attr |6| |Data security integrity|) missing))
(assert (= (state-attr |6| |Data Store|) missing))
(assert (= (state-attr |6| |DDoS Mitigation|) missing))
(assert (= (state-attr |6| |Digital Signature|) missing))
(assert (= (state-attr |6| Encryption) missing))
(assert (= (state-attr |6| |Encryption Method|) missing))
(assert (= (state-attr |6| |Encryption Time|) missing))
(assert (= (state-attr |6| |Error Rate|) missing))
(assert (= (state-attr |6| Feedback) missing))
(assert (= (state-attr |6| |Financial Asset|) missing))
(assert (= (state-attr |6| Firmware) missing))
(assert (= (state-attr |6| |Input Validation|) missing))
(assert (= (state-attr |6| Integrity) missing))
(assert (= (state-attr |6| |Key Length|) missing))
(assert (= (state-attr |6| |Key Revocation|) missing))
(assert (= (state-attr |6| Language) missing))
(assert (= (state-attr |6| License) missing))
(assert (= (state-attr |6| Location) missing))
(assert (= (state-attr |6| |Maximum Value|) missing))
(assert (= (state-attr |6| |Memory Type|) missing))
(assert (= (state-attr |6| |Minimum Value|) missing))
(assert (= (state-attr |6| |Network Technology|) missing))
(assert (= (state-attr |6| |Operating system|) missing))
(assert (= (state-attr |6| |Operational Criticality|) missing))
(assert (= (state-attr |6| Permissions) missing))
(assert (= (state-attr |6| |Physical Location|) missing))
(assert (= (state-attr |6| |Power consumption|) missing))
(assert (= (state-attr |6| |Privacy Asset|) missing))
(assert (= (state-attr |6| |Processing Time|) missing))
(assert (= (state-attr |6| |Protocol version|) missing))
(assert (= (state-attr |6| Protocols) missing))
(assert (= (state-attr |6| |PtwoP Capability|) missing))
(assert (= (state-attr |6| Range) missing))
(assert (= (state-attr |6| Redundancy) missing))
(assert (= (state-attr |6| |Reset capabilities|) missing))
(assert (= (state-attr |6| Roles) missing))
(assert (= (state-attr |6| |Secure Boot|) missing))
(assert (= (state-attr |6| |Secure Session Handling|) missing))
(assert (= (state-attr |6| |Secure Storage|) missing))
(assert (= (state-attr |6| |Secure Update|) missing))
(assert (= (state-attr |6| |Sensor measurement type|) missing))
(assert (= (state-attr |6| |Shared resources|) missing))
(assert (= (state-attr |6| Software) missing))
(assert (= (state-attr |6| |Software APIs|) missing))
(assert (= (state-attr |6| Storage) missing))
(assert (= (state-attr |6| |Token Signing|) missing))
(assert (= (state-attr |6| Troughput) missing))
(assert (= (state-attr |6| Unit) missing))
(assert (= (state-attr |6| |Update capabilities|) missing))
(assert (= (state-attr |6| Updates) missing))
(assert (= (state-attr |6| |URL Blacklisting|) missing))
(assert (= (state-attr |6| |User File Upload|) missing))
(assert (= (state-attr |6| |User Interfaces|) missing))
(assert (= (state-attr |6| |User Management|) missing))
(assert (= (state-attr |6| |Wired interface|) missing))
(assert (= (state-attr |6| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |6| |Wireless Interface|) missing))
(assert (= (is-boundary |10|) false))
(assert (= (state-type |10|) |IoT Device|))
(assert (or (= (state-attr |10| |Allows User Input|) undefined)
    (= (state-attr |10| |Allows User Input|) Yes)
    (= (state-attr |10| |Allows User Input|) No)
    (= (state-attr |10| |Allows User Input|) undefined)
    (= (state-attr |10| |Allows User Input|) Yes)
    (= (state-attr |10| |Allows User Input|) No)
    (= (state-attr |10| |Allows User Input|) undefined)
    (= (state-attr |10| |Allows User Input|) Yes)
    (= (state-attr |10| |Allows User Input|) No)))
(assert (or (= (state-attr |10| |Approved License|) undefined)
    (= (state-attr |10| |Approved License|) Yes)
    (= (state-attr |10| |Approved License|) No)
    (= (state-attr |10| |Approved License|) undefined)
    (= (state-attr |10| |Approved License|) Yes)
    (= (state-attr |10| |Approved License|) No)
    (= (state-attr |10| |Approved License|) undefined)
    (= (state-attr |10| |Approved License|) Yes)
    (= (state-attr |10| |Approved License|) No)))
(assert (or (= (state-attr |10| Authentication) undefined)
    (= (state-attr |10| Authentication) strong)
    (= (state-attr |10| Authentication) Yes)
    (= (state-attr |10| Authentication) No)
    (= (state-attr |10| Authentication) undefined)
    (= (state-attr |10| Authentication) strong)
    (= (state-attr |10| Authentication) Yes)
    (= (state-attr |10| Authentication) No)
    (= (state-attr |10| Authentication) undefined)
    (= (state-attr |10| Authentication) strong)
    (= (state-attr |10| Authentication) Yes)
    (= (state-attr |10| Authentication) No)))
(assert (or (= (state-attr |10| Authorization) undefined)
    (= (state-attr |10| Authorization) strong)
    (= (state-attr |10| Authorization) Yes)
    (= (state-attr |10| Authorization) No)
    (= (state-attr |10| Authorization) undefined)
    (= (state-attr |10| Authorization) strong)
    (= (state-attr |10| Authorization) Yes)
    (= (state-attr |10| Authorization) No)
    (= (state-attr |10| Authorization) undefined)
    (= (state-attr |10| Authorization) strong)
    (= (state-attr |10| Authorization) Yes)
    (= (state-attr |10| Authorization) No)))
(assert (or (= (state-attr |10| |Certificate Checks|) undefined)
    (= (state-attr |10| |Certificate Checks|) Yes)
    (= (state-attr |10| |Certificate Checks|) No)
    (= (state-attr |10| |Certificate Checks|) undefined)
    (= (state-attr |10| |Certificate Checks|) Yes)
    (= (state-attr |10| |Certificate Checks|) No)
    (= (state-attr |10| |Certificate Checks|) undefined)
    (= (state-attr |10| |Certificate Checks|) Yes)
    (= (state-attr |10| |Certificate Checks|) No)))
(assert (or (= (state-attr |10| |Counterfeit Detection|) undefined)
    (= (state-attr |10| |Counterfeit Detection|) No)
    (= (state-attr |10| |Counterfeit Detection|) Yes)
    (= (state-attr |10| |Counterfeit Detection|) undefined)
    (= (state-attr |10| |Counterfeit Detection|) No)
    (= (state-attr |10| |Counterfeit Detection|) Yes)
    (= (state-attr |10| |Counterfeit Detection|) undefined)
    (= (state-attr |10| |Counterfeit Detection|) No)
    (= (state-attr |10| |Counterfeit Detection|) Yes)))
(assert (or (= (state-attr |10| |Cryptographic Hardware|) undefined)
    (= (state-attr |10| |Cryptographic Hardware|) Yes)
    (= (state-attr |10| |Cryptographic Hardware|) No)
    (= (state-attr |10| |Cryptographic Hardware|) undefined)
    (= (state-attr |10| |Cryptographic Hardware|) Yes)
    (= (state-attr |10| |Cryptographic Hardware|) No)
    (= (state-attr |10| |Cryptographic Hardware|) undefined)
    (= (state-attr |10| |Cryptographic Hardware|) Yes)
    (= (state-attr |10| |Cryptographic Hardware|) No)))
(assert (or (= (state-attr |10| Encrypted) undefined)
    (= (state-attr |10| Encrypted) Yes)
    (= (state-attr |10| Encrypted) No)
    (= (state-attr |10| Encrypted) strong)
    (= (state-attr |10| Encrypted) undefined)
    (= (state-attr |10| Encrypted) Yes)
    (= (state-attr |10| Encrypted) No)
    (= (state-attr |10| Encrypted) strong)
    (= (state-attr |10| Encrypted) undefined)
    (= (state-attr |10| Encrypted) Yes)
    (= (state-attr |10| Encrypted) No)
    (= (state-attr |10| Encrypted) strong)))
(assert (or (= (state-attr |10| |Encryption Method|) undefined)
    (= (state-attr |10| |Encryption Method|) strong)
    (= (state-attr |10| |Encryption Method|) weak)
    (= (state-attr |10| |Encryption Method|) undefined)
    (= (state-attr |10| |Encryption Method|) strong)
    (= (state-attr |10| |Encryption Method|) weak)
    (= (state-attr |10| |Encryption Method|) undefined)
    (= (state-attr |10| |Encryption Method|) strong)
    (= (state-attr |10| |Encryption Method|) weak)))
(assert (or (= (state-attr |10| |Financial Asset|) undefined)
    (= (state-attr |10| |Financial Asset|) Yes)
    (= (state-attr |10| |Financial Asset|) No)
    (= (state-attr |10| |Financial Asset|) undefined)
    (= (state-attr |10| |Financial Asset|) Yes)
    (= (state-attr |10| |Financial Asset|) No)
    (= (state-attr |10| |Financial Asset|) undefined)
    (= (state-attr |10| |Financial Asset|) Yes)
    (= (state-attr |10| |Financial Asset|) No)))
(assert (or (= (state-attr |10| Location) undefined)
    (= (state-attr |10| Location) |On Premise|)
    (= (state-attr |10| Location) |Off Premise|)
    (= (state-attr |10| Location) Cloud)
    (= (state-attr |10| Location) Mobile)
    (= (state-attr |10| Location) undefined)
    (= (state-attr |10| Location) |On Premise|)
    (= (state-attr |10| Location) |Off Premise|)
    (= (state-attr |10| Location) Cloud)
    (= (state-attr |10| Location) Mobile)
    (= (state-attr |10| Location) undefined)
    (= (state-attr |10| Location) |On Premise|)
    (= (state-attr |10| Location) |Off Premise|)
    (= (state-attr |10| Location) Cloud)
    (= (state-attr |10| Location) Mobile)))
(assert (or (= (state-attr |10| |Malware Protection|) undefined)
    (= (state-attr |10| |Malware Protection|) Yes)
    (= (state-attr |10| |Malware Protection|) No)
    (= (state-attr |10| |Malware Protection|) undefined)
    (= (state-attr |10| |Malware Protection|) Yes)
    (= (state-attr |10| |Malware Protection|) No)
    (= (state-attr |10| |Malware Protection|) undefined)
    (= (state-attr |10| |Malware Protection|) Yes)
    (= (state-attr |10| |Malware Protection|) No)))
(assert (or (= (state-attr |10| Managed) undefined)
    (= (state-attr |10| Managed) No)
    (= (state-attr |10| Managed) Yes)
    (= (state-attr |10| Managed) undefined)
    (= (state-attr |10| Managed) No)
    (= (state-attr |10| Managed) Yes)
    (= (state-attr |10| Managed) undefined)
    (= (state-attr |10| Managed) No)
    (= (state-attr |10| Managed) Yes)))
(assert (or (= (state-attr |10| |Privacy Asset|) undefined)
    (= (state-attr |10| |Privacy Asset|) Yes)
    (= (state-attr |10| |Privacy Asset|) No)
    (= (state-attr |10| |Privacy Asset|) multiple)
    (= (state-attr |10| |Privacy Asset|) undefined)
    (= (state-attr |10| |Privacy Asset|) Yes)
    (= (state-attr |10| |Privacy Asset|) No)
    (= (state-attr |10| |Privacy Asset|) multiple)
    (= (state-attr |10| |Privacy Asset|) undefined)
    (= (state-attr |10| |Privacy Asset|) Yes)
    (= (state-attr |10| |Privacy Asset|) No)
    (= (state-attr |10| |Privacy Asset|) multiple)))
(assert (or (= (state-attr |10| |Protected Execution Environment|) undefined)
    (= (state-attr |10| |Protected Execution Environment|) Yes)
    (= (state-attr |10| |Protected Execution Environment|) No)
    (= (state-attr |10| |Protected Execution Environment|) undefined)
    (= (state-attr |10| |Protected Execution Environment|) Yes)
    (= (state-attr |10| |Protected Execution Environment|) No)
    (= (state-attr |10| |Protected Execution Environment|) undefined)
    (= (state-attr |10| |Protected Execution Environment|) Yes)
    (= (state-attr |10| |Protected Execution Environment|) No)))
(assert (or (= (state-attr |10| |PtwoP Capability|) undefined)
    (= (state-attr |10| |PtwoP Capability|) Yes)
    (= (state-attr |10| |PtwoP Capability|) No)
    (= (state-attr |10| |PtwoP Capability|) undefined)
    (= (state-attr |10| |PtwoP Capability|) Yes)
    (= (state-attr |10| |PtwoP Capability|) No)
    (= (state-attr |10| |PtwoP Capability|) undefined)
    (= (state-attr |10| |PtwoP Capability|) Yes)
    (= (state-attr |10| |PtwoP Capability|) No)))
(assert (or (= (state-attr |10| |Secure Session Handling|) undefined)
    (= (state-attr |10| |Secure Session Handling|) Yes)
    (= (state-attr |10| |Secure Session Handling|) No)
    (= (state-attr |10| |Secure Session Handling|) undefined)
    (= (state-attr |10| |Secure Session Handling|) Yes)
    (= (state-attr |10| |Secure Session Handling|) No)
    (= (state-attr |10| |Secure Session Handling|) undefined)
    (= (state-attr |10| |Secure Session Handling|) Yes)
    (= (state-attr |10| |Secure Session Handling|) No)))
(assert (or (= (state-attr |10| |Standard Password|) undefined)
    (= (state-attr |10| |Standard Password|) Yes)
    (= (state-attr |10| |Standard Password|) No)
    (= (state-attr |10| |Standard Password|) undefined)
    (= (state-attr |10| |Standard Password|) Yes)
    (= (state-attr |10| |Standard Password|) No)
    (= (state-attr |10| |Standard Password|) undefined)
    (= (state-attr |10| |Standard Password|) Yes)
    (= (state-attr |10| |Standard Password|) No)))
(assert (or (= (state-attr |10| Storage) undefined)
    (= (state-attr |10| Storage) Removeable)
    (= (state-attr |10| Storage) undefined)
    (= (state-attr |10| Storage) Removeable)
    (= (state-attr |10| Storage) undefined)
    (= (state-attr |10| Storage) Removeable)))
(assert (or (= (state-attr |10| |Tamper Protection|) Yes)
    (= (state-attr |10| |Tamper Protection|) No)
    (= (state-attr |10| |Tamper Protection|) undefined)))
(assert (or (= (state-attr |10| |Token Signing|) undefined)
    (= (state-attr |10| |Token Signing|) Yes)
    (= (state-attr |10| |Token Signing|) No)
    (= (state-attr |10| |Token Signing|) undefined)
    (= (state-attr |10| |Token Signing|) Yes)
    (= (state-attr |10| |Token Signing|) No)
    (= (state-attr |10| |Token Signing|) undefined)
    (= (state-attr |10| |Token Signing|) Yes)
    (= (state-attr |10| |Token Signing|) No)))
(assert (or (= (state-attr |10| |URL Blacklisting|) undefined)
    (= (state-attr |10| |URL Blacklisting|) Yes)
    (= (state-attr |10| |URL Blacklisting|) No)
    (= (state-attr |10| |URL Blacklisting|) undefined)
    (= (state-attr |10| |URL Blacklisting|) Yes)
    (= (state-attr |10| |URL Blacklisting|) No)
    (= (state-attr |10| |URL Blacklisting|) undefined)
    (= (state-attr |10| |URL Blacklisting|) Yes)
    (= (state-attr |10| |URL Blacklisting|) No)))
(assert (= (state-attr |10| |Access Control|) missing))
(assert (= (state-attr |10| |Activity Logging|) missing))
(assert (= (state-attr |10| Administration) missing))
(assert (= (state-attr |10| |Anomaly Detection|) missing))
(assert (= (state-attr |10| |API Type|) missing))
(assert (= (state-attr |10| Auditing) missing))
(assert (= (state-attr |10| Availability) missing))
(assert (= (state-attr |10| Bandwidth) missing))
(assert (= (state-attr |10| |Coding guideline|) missing))
(assert (= (state-attr |10| |Communication Latency|) missing))
(assert (= (state-attr |10| |Communication Reliability|) missing))
(assert (= (state-attr |10| Confidentiality) missing))
(assert (= (state-attr |10| Content) missing))
(assert (= (state-attr |10| |Credential Asset|) missing))
(assert (= (state-attr |10| Criticality) missing))
(assert (= (state-attr |10| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |10| |Data Backup|) missing))
(assert (= (state-attr |10| |Data safety integrity|) missing))
(assert (= (state-attr |10| |Data security integrity|) missing))
(assert (= (state-attr |10| |Data Store|) missing))
(assert (= (state-attr |10| |DDoS Mitigation|) missing))
(assert (= (state-attr |10| |Device Fingerprint|) missing))
(assert (= (state-attr |10| |Digital Signature|) missing))
(assert (= (state-attr |10| Encryption) missing))
(assert (= (state-attr |10| |Encryption Time|) missing))
(assert (= (state-attr |10| |Error Rate|) missing))
(assert (= (state-attr |10| Feedback) missing))
(assert (= (state-attr |10| Firmware) missing))
(assert (= (state-attr |10| |Input Sanitization|) missing))
(assert (= (state-attr |10| |Input Validation|) missing))
(assert (= (state-attr |10| Integrity) missing))
(assert (= (state-attr |10| |Key Length|) missing))
(assert (= (state-attr |10| |Key Revocation|) missing))
(assert (= (state-attr |10| Language) missing))
(assert (= (state-attr |10| License) missing))
(assert (= (state-attr |10| |Maximum Value|) missing))
(assert (= (state-attr |10| |Memory Type|) missing))
(assert (= (state-attr |10| |Minimum Value|) missing))
(assert (= (state-attr |10| |Network Technology|) missing))
(assert (= (state-attr |10| |Operating system|) missing))
(assert (= (state-attr |10| |Operational Criticality|) missing))
(assert (= (state-attr |10| Permissions) missing))
(assert (= (state-attr |10| |Physical Location|) missing))
(assert (= (state-attr |10| |Power consumption|) missing))
(assert (= (state-attr |10| |Processing Time|) missing))
(assert (= (state-attr |10| |Protocol version|) missing))
(assert (= (state-attr |10| Protocols) missing))
(assert (= (state-attr |10| Range) missing))
(assert (= (state-attr |10| Redundancy) missing))
(assert (= (state-attr |10| |Reset capabilities|) missing))
(assert (= (state-attr |10| Roles) missing))
(assert (= (state-attr |10| |Secure Boot|) missing))
(assert (= (state-attr |10| |Secure Storage|) missing))
(assert (= (state-attr |10| |Secure Update|) missing))
(assert (= (state-attr |10| |Sensor measurement type|) missing))
(assert (= (state-attr |10| |Shared resources|) missing))
(assert (= (state-attr |10| Software) missing))
(assert (= (state-attr |10| |Software APIs|) missing))
(assert (= (state-attr |10| |Token Validation|) missing))
(assert (= (state-attr |10| Troughput) missing))
(assert (= (state-attr |10| Unit) missing))
(assert (= (state-attr |10| |Update capabilities|) missing))
(assert (= (state-attr |10| Updates) missing))
(assert (= (state-attr |10| |User File Upload|) missing))
(assert (= (state-attr |10| |User Interfaces|) missing))
(assert (= (state-attr |10| |User Management|) missing))
(assert (= (state-attr |10| |Wired interface|) missing))
(assert (= (state-attr |10| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |10| |Wireless Interface|) missing))
(assert (= (is-boundary |12|) false))
(assert (= (state-type |12|) |Web Server|))
(assert (or (= (state-attr |12| |Activity Logging|) undefined)
    (= (state-attr |12| |Activity Logging|) Yes)
    (= (state-attr |12| |Activity Logging|) No)
    (= (state-attr |12| |Activity Logging|) undefined)
    (= (state-attr |12| |Activity Logging|) Yes)
    (= (state-attr |12| |Activity Logging|) No)
    (= (state-attr |12| |Activity Logging|) undefined)
    (= (state-attr |12| |Activity Logging|) Yes)
    (= (state-attr |12| |Activity Logging|) No)))
(assert (or (= (state-attr |12| |Allows User Input|) undefined)
    (= (state-attr |12| |Allows User Input|) Yes)
    (= (state-attr |12| |Allows User Input|) No)
    (= (state-attr |12| |Allows User Input|) undefined)
    (= (state-attr |12| |Allows User Input|) Yes)
    (= (state-attr |12| |Allows User Input|) No)
    (= (state-attr |12| |Allows User Input|) undefined)
    (= (state-attr |12| |Allows User Input|) Yes)
    (= (state-attr |12| |Allows User Input|) No)))
(assert (or (= (state-attr |12| |Anomaly Detection|) undefined)
    (= (state-attr |12| |Anomaly Detection|) Yes)
    (= (state-attr |12| |Anomaly Detection|) No)
    (= (state-attr |12| |Anomaly Detection|) undefined)
    (= (state-attr |12| |Anomaly Detection|) Yes)
    (= (state-attr |12| |Anomaly Detection|) No)
    (= (state-attr |12| |Anomaly Detection|) undefined)
    (= (state-attr |12| |Anomaly Detection|) Yes)
    (= (state-attr |12| |Anomaly Detection|) No)))
(assert (or (= (state-attr |12| Authentication) undefined)
    (= (state-attr |12| Authentication) strong)
    (= (state-attr |12| Authentication) Yes)
    (= (state-attr |12| Authentication) No)
    (= (state-attr |12| Authentication) undefined)
    (= (state-attr |12| Authentication) strong)
    (= (state-attr |12| Authentication) Yes)
    (= (state-attr |12| Authentication) No)
    (= (state-attr |12| Authentication) undefined)
    (= (state-attr |12| Authentication) strong)
    (= (state-attr |12| Authentication) Yes)
    (= (state-attr |12| Authentication) No)))
(assert (or (= (state-attr |12| Authorization) undefined)
    (= (state-attr |12| Authorization) strong)
    (= (state-attr |12| Authorization) Yes)
    (= (state-attr |12| Authorization) No)
    (= (state-attr |12| Authorization) undefined)
    (= (state-attr |12| Authorization) strong)
    (= (state-attr |12| Authorization) Yes)
    (= (state-attr |12| Authorization) No)
    (= (state-attr |12| Authorization) undefined)
    (= (state-attr |12| Authorization) strong)
    (= (state-attr |12| Authorization) Yes)
    (= (state-attr |12| Authorization) No)))
(assert (or (= (state-attr |12| |DDoS Mitigation|) undefined)
    (= (state-attr |12| |DDoS Mitigation|) Yes)
    (= (state-attr |12| |DDoS Mitigation|) No)
    (= (state-attr |12| |DDoS Mitigation|) undefined)
    (= (state-attr |12| |DDoS Mitigation|) Yes)
    (= (state-attr |12| |DDoS Mitigation|) No)
    (= (state-attr |12| |DDoS Mitigation|) undefined)
    (= (state-attr |12| |DDoS Mitigation|) Yes)
    (= (state-attr |12| |DDoS Mitigation|) No)))
(assert (or (= (state-attr |12| Encrypted) undefined)
    (= (state-attr |12| Encrypted) Yes)
    (= (state-attr |12| Encrypted) No)
    (= (state-attr |12| Encrypted) strong)
    (= (state-attr |12| Encrypted) undefined)
    (= (state-attr |12| Encrypted) Yes)
    (= (state-attr |12| Encrypted) No)
    (= (state-attr |12| Encrypted) strong)
    (= (state-attr |12| Encrypted) undefined)
    (= (state-attr |12| Encrypted) Yes)
    (= (state-attr |12| Encrypted) No)
    (= (state-attr |12| Encrypted) strong)))
(assert (or (= (state-attr |12| |Key Revocation|) undefined)
    (= (state-attr |12| |Key Revocation|) Yes)
    (= (state-attr |12| |Key Revocation|) No)
    (= (state-attr |12| |Key Revocation|) undefined)
    (= (state-attr |12| |Key Revocation|) Yes)
    (= (state-attr |12| |Key Revocation|) No)
    (= (state-attr |12| |Key Revocation|) undefined)
    (= (state-attr |12| |Key Revocation|) Yes)
    (= (state-attr |12| |Key Revocation|) No)))
(assert (or (= (state-attr |12| Location) undefined)
    (= (state-attr |12| Location) |On Premise|)
    (= (state-attr |12| Location) |Off Premise|)
    (= (state-attr |12| Location) Cloud)
    (= (state-attr |12| Location) Mobile)
    (= (state-attr |12| Location) undefined)
    (= (state-attr |12| Location) |On Premise|)
    (= (state-attr |12| Location) |Off Premise|)
    (= (state-attr |12| Location) Cloud)
    (= (state-attr |12| Location) Mobile)
    (= (state-attr |12| Location) undefined)
    (= (state-attr |12| Location) |On Premise|)
    (= (state-attr |12| Location) |Off Premise|)
    (= (state-attr |12| Location) Cloud)
    (= (state-attr |12| Location) Mobile)))
(assert (or (= (state-attr |12| Managed) undefined)
    (= (state-attr |12| Managed) No)
    (= (state-attr |12| Managed) Yes)
    (= (state-attr |12| Managed) undefined)
    (= (state-attr |12| Managed) No)
    (= (state-attr |12| Managed) Yes)
    (= (state-attr |12| Managed) undefined)
    (= (state-attr |12| Managed) No)
    (= (state-attr |12| Managed) Yes)))
(assert (or (= (state-attr |12| |Protected Execution Environment|) undefined)
    (= (state-attr |12| |Protected Execution Environment|) Yes)
    (= (state-attr |12| |Protected Execution Environment|) No)
    (= (state-attr |12| |Protected Execution Environment|) undefined)
    (= (state-attr |12| |Protected Execution Environment|) Yes)
    (= (state-attr |12| |Protected Execution Environment|) No)
    (= (state-attr |12| |Protected Execution Environment|) undefined)
    (= (state-attr |12| |Protected Execution Environment|) Yes)
    (= (state-attr |12| |Protected Execution Environment|) No)))
(assert (or (= (state-attr |12| Roles) undefined)
    (= (state-attr |12| Roles) admin)
    (= (state-attr |12| Roles) user)
    (= (state-attr |12| Roles) manager)
    (= (state-attr |12| Roles) operator)
    (= (state-attr |12| Roles) undefined)
    (= (state-attr |12| Roles) admin)
    (= (state-attr |12| Roles) user)
    (= (state-attr |12| Roles) manager)
    (= (state-attr |12| Roles) operator)
    (= (state-attr |12| Roles) undefined)
    (= (state-attr |12| Roles) admin)
    (= (state-attr |12| Roles) user)
    (= (state-attr |12| Roles) manager)
    (= (state-attr |12| Roles) operator)))
(assert (or (= (state-attr |12| |Tamper Protection|) Yes)
    (= (state-attr |12| |Tamper Protection|) No)
    (= (state-attr |12| |Tamper Protection|) undefined)))
(assert (or (= (state-attr |12| |Token Validation|) undefined)
    (= (state-attr |12| |Token Validation|) Yes)
    (= (state-attr |12| |Token Validation|) No)
    (= (state-attr |12| |Token Validation|) undefined)
    (= (state-attr |12| |Token Validation|) Yes)
    (= (state-attr |12| |Token Validation|) No)
    (= (state-attr |12| |Token Validation|) undefined)
    (= (state-attr |12| |Token Validation|) Yes)
    (= (state-attr |12| |Token Validation|) No)))
(assert (= (state-attr |12| |Access Control|) missing))
(assert (= (state-attr |12| Administration) missing))
(assert (= (state-attr |12| |API Type|) missing))
(assert (= (state-attr |12| |Approved License|) missing))
(assert (= (state-attr |12| Auditing) missing))
(assert (= (state-attr |12| Availability) missing))
(assert (= (state-attr |12| Bandwidth) missing))
(assert (= (state-attr |12| |Certificate Checks|) missing))
(assert (= (state-attr |12| |Coding guideline|) missing))
(assert (= (state-attr |12| |Communication Latency|) missing))
(assert (= (state-attr |12| |Communication Reliability|) missing))
(assert (= (state-attr |12| Confidentiality) missing))
(assert (= (state-attr |12| Content) missing))
(assert (= (state-attr |12| |Counterfeit Detection|) missing))
(assert (= (state-attr |12| |Credential Asset|) missing))
(assert (= (state-attr |12| Criticality) missing))
(assert (= (state-attr |12| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |12| |Cryptographic Hardware|) missing))
(assert (= (state-attr |12| |Data Backup|) missing))
(assert (= (state-attr |12| |Data safety integrity|) missing))
(assert (= (state-attr |12| |Data security integrity|) missing))
(assert (= (state-attr |12| |Data Store|) missing))
(assert (= (state-attr |12| |Device Fingerprint|) missing))
(assert (= (state-attr |12| |Digital Signature|) missing))
(assert (= (state-attr |12| Encryption) missing))
(assert (= (state-attr |12| |Encryption Method|) missing))
(assert (= (state-attr |12| |Encryption Time|) missing))
(assert (= (state-attr |12| |Error Rate|) missing))
(assert (= (state-attr |12| Feedback) missing))
(assert (= (state-attr |12| |Financial Asset|) missing))
(assert (= (state-attr |12| Firmware) missing))
(assert (= (state-attr |12| |Input Sanitization|) missing))
(assert (= (state-attr |12| |Input Validation|) missing))
(assert (= (state-attr |12| Integrity) missing))
(assert (= (state-attr |12| |Key Length|) missing))
(assert (= (state-attr |12| Language) missing))
(assert (= (state-attr |12| License) missing))
(assert (= (state-attr |12| |Malware Protection|) missing))
(assert (= (state-attr |12| |Maximum Value|) missing))
(assert (= (state-attr |12| |Memory Type|) missing))
(assert (= (state-attr |12| |Minimum Value|) missing))
(assert (= (state-attr |12| |Network Technology|) missing))
(assert (= (state-attr |12| |Operating system|) missing))
(assert (= (state-attr |12| |Operational Criticality|) missing))
(assert (= (state-attr |12| Permissions) missing))
(assert (= (state-attr |12| |Physical Location|) missing))
(assert (= (state-attr |12| |Power consumption|) missing))
(assert (= (state-attr |12| |Privacy Asset|) missing))
(assert (= (state-attr |12| |Processing Time|) missing))
(assert (= (state-attr |12| |Protocol version|) missing))
(assert (= (state-attr |12| Protocols) missing))
(assert (= (state-attr |12| |PtwoP Capability|) missing))
(assert (= (state-attr |12| Range) missing))
(assert (= (state-attr |12| Redundancy) missing))
(assert (= (state-attr |12| |Reset capabilities|) missing))
(assert (= (state-attr |12| |Secure Boot|) missing))
(assert (= (state-attr |12| |Secure Session Handling|) missing))
(assert (= (state-attr |12| |Secure Storage|) missing))
(assert (= (state-attr |12| |Secure Update|) missing))
(assert (= (state-attr |12| |Sensor measurement type|) missing))
(assert (= (state-attr |12| |Shared resources|) missing))
(assert (= (state-attr |12| Software) missing))
(assert (= (state-attr |12| |Software APIs|) missing))
(assert (= (state-attr |12| |Standard Password|) missing))
(assert (= (state-attr |12| Storage) missing))
(assert (= (state-attr |12| |Token Signing|) missing))
(assert (= (state-attr |12| Troughput) missing))
(assert (= (state-attr |12| Unit) missing))
(assert (= (state-attr |12| |Update capabilities|) missing))
(assert (= (state-attr |12| Updates) missing))
(assert (= (state-attr |12| |URL Blacklisting|) missing))
(assert (= (state-attr |12| |User File Upload|) missing))
(assert (= (state-attr |12| |User Interfaces|) missing))
(assert (= (state-attr |12| |User Management|) missing))
(assert (= (state-attr |12| |Wired interface|) missing))
(assert (= (state-attr |12| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |12| |Wireless Interface|) missing))
(assert (= (is-boundary |46|) false))
(assert (= (state-type |46|) Firewall))
(assert (or (= (state-attr |46| |Activity Logging|) undefined)
    (= (state-attr |46| |Activity Logging|) Yes)
    (= (state-attr |46| |Activity Logging|) No)
    (= (state-attr |46| |Activity Logging|) undefined)
    (= (state-attr |46| |Activity Logging|) Yes)
    (= (state-attr |46| |Activity Logging|) No)
    (= (state-attr |46| |Activity Logging|) undefined)
    (= (state-attr |46| |Activity Logging|) Yes)
    (= (state-attr |46| |Activity Logging|) No)))
(assert (or (= (state-attr |46| Authentication) undefined)
    (= (state-attr |46| Authentication) strong)
    (= (state-attr |46| Authentication) Yes)
    (= (state-attr |46| Authentication) No)
    (= (state-attr |46| Authentication) undefined)
    (= (state-attr |46| Authentication) strong)
    (= (state-attr |46| Authentication) Yes)
    (= (state-attr |46| Authentication) No)
    (= (state-attr |46| Authentication) undefined)
    (= (state-attr |46| Authentication) strong)
    (= (state-attr |46| Authentication) Yes)
    (= (state-attr |46| Authentication) No)))
(assert (or (= (state-attr |46| Authorization) undefined)
    (= (state-attr |46| Authorization) strong)
    (= (state-attr |46| Authorization) Yes)
    (= (state-attr |46| Authorization) No)
    (= (state-attr |46| Authorization) undefined)
    (= (state-attr |46| Authorization) strong)
    (= (state-attr |46| Authorization) Yes)
    (= (state-attr |46| Authorization) No)
    (= (state-attr |46| Authorization) undefined)
    (= (state-attr |46| Authorization) strong)
    (= (state-attr |46| Authorization) Yes)
    (= (state-attr |46| Authorization) No)))
(assert (or (= (state-attr |46| |DDoS Mitigation|) undefined)
    (= (state-attr |46| |DDoS Mitigation|) Yes)
    (= (state-attr |46| |DDoS Mitigation|) No)
    (= (state-attr |46| |DDoS Mitigation|) undefined)
    (= (state-attr |46| |DDoS Mitigation|) Yes)
    (= (state-attr |46| |DDoS Mitigation|) No)
    (= (state-attr |46| |DDoS Mitigation|) undefined)
    (= (state-attr |46| |DDoS Mitigation|) Yes)
    (= (state-attr |46| |DDoS Mitigation|) No)))
(assert (= (state-attr |46| |Access Control|) missing))
(assert (= (state-attr |46| Administration) missing))
(assert (= (state-attr |46| |Allows User Input|) missing))
(assert (= (state-attr |46| |Anomaly Detection|) missing))
(assert (= (state-attr |46| |API Type|) missing))
(assert (= (state-attr |46| |Approved License|) missing))
(assert (= (state-attr |46| Auditing) missing))
(assert (= (state-attr |46| Availability) missing))
(assert (= (state-attr |46| Bandwidth) missing))
(assert (= (state-attr |46| |Certificate Checks|) missing))
(assert (= (state-attr |46| |Coding guideline|) missing))
(assert (= (state-attr |46| |Communication Latency|) missing))
(assert (= (state-attr |46| |Communication Reliability|) missing))
(assert (= (state-attr |46| Confidentiality) missing))
(assert (= (state-attr |46| Content) missing))
(assert (= (state-attr |46| |Counterfeit Detection|) missing))
(assert (= (state-attr |46| |Credential Asset|) missing))
(assert (= (state-attr |46| Criticality) missing))
(assert (= (state-attr |46| |Cryptographic Algorithms|) missing))
(assert (= (state-attr |46| |Cryptographic Hardware|) missing))
(assert (= (state-attr |46| |Data Backup|) missing))
(assert (= (state-attr |46| |Data safety integrity|) missing))
(assert (= (state-attr |46| |Data security integrity|) missing))
(assert (= (state-attr |46| |Data Store|) missing))
(assert (= (state-attr |46| |Device Fingerprint|) missing))
(assert (= (state-attr |46| |Digital Signature|) missing))
(assert (= (state-attr |46| Encrypted) missing))
(assert (= (state-attr |46| Encryption) missing))
(assert (= (state-attr |46| |Encryption Method|) missing))
(assert (= (state-attr |46| |Encryption Time|) missing))
(assert (= (state-attr |46| |Error Rate|) missing))
(assert (= (state-attr |46| Feedback) missing))
(assert (= (state-attr |46| |Financial Asset|) missing))
(assert (= (state-attr |46| Firmware) missing))
(assert (= (state-attr |46| |Input Sanitization|) missing))
(assert (= (state-attr |46| |Input Validation|) missing))
(assert (= (state-attr |46| Integrity) missing))
(assert (= (state-attr |46| |Key Length|) missing))
(assert (= (state-attr |46| |Key Revocation|) missing))
(assert (= (state-attr |46| Language) missing))
(assert (= (state-attr |46| License) missing))
(assert (= (state-attr |46| Location) missing))
(assert (= (state-attr |46| |Malware Protection|) missing))
(assert (= (state-attr |46| Managed) missing))
(assert (= (state-attr |46| |Maximum Value|) missing))
(assert (= (state-attr |46| |Memory Type|) missing))
(assert (= (state-attr |46| |Minimum Value|) missing))
(assert (= (state-attr |46| |Network Technology|) missing))
(assert (= (state-attr |46| |Operating system|) missing))
(assert (= (state-attr |46| |Operational Criticality|) missing))
(assert (= (state-attr |46| Permissions) missing))
(assert (= (state-attr |46| |Physical Location|) missing))
(assert (= (state-attr |46| |Power consumption|) missing))
(assert (= (state-attr |46| |Privacy Asset|) missing))
(assert (= (state-attr |46| |Processing Time|) missing))
(assert (= (state-attr |46| |Protected Execution Environment|) missing))
(assert (= (state-attr |46| |Protocol version|) missing))
(assert (= (state-attr |46| Protocols) missing))
(assert (= (state-attr |46| |PtwoP Capability|) missing))
(assert (= (state-attr |46| Range) missing))
(assert (= (state-attr |46| Redundancy) missing))
(assert (= (state-attr |46| |Reset capabilities|) missing))
(assert (= (state-attr |46| Roles) missing))
(assert (= (state-attr |46| |Secure Boot|) missing))
(assert (= (state-attr |46| |Secure Session Handling|) missing))
(assert (= (state-attr |46| |Secure Storage|) missing))
(assert (= (state-attr |46| |Secure Update|) missing))
(assert (= (state-attr |46| |Sensor measurement type|) missing))
(assert (= (state-attr |46| |Shared resources|) missing))
(assert (= (state-attr |46| Software) missing))
(assert (= (state-attr |46| |Software APIs|) missing))
(assert (= (state-attr |46| |Standard Password|) missing))
(assert (= (state-attr |46| Storage) missing))
(assert (= (state-attr |46| |Tamper Protection|) missing))
(assert (= (state-attr |46| |Token Signing|) missing))
(assert (= (state-attr |46| |Token Validation|) missing))
(assert (= (state-attr |46| Troughput) missing))
(assert (= (state-attr |46| Unit) missing))
(assert (= (state-attr |46| |Update capabilities|) missing))
(assert (= (state-attr |46| Updates) missing))
(assert (= (state-attr |46| |URL Blacklisting|) missing))
(assert (= (state-attr |46| |User File Upload|) missing))
(assert (= (state-attr |46| |User Interfaces|) missing))
(assert (= (state-attr |46| |User Management|) missing))
(assert (= (state-attr |46| |Wired interface|) missing))
(assert (= (state-attr |46| |Wireless Communication Technologie|) missing))
(assert (= (state-attr |46| |Wireless Interface|) missing))
(assert (= (is-boundary |47|) true))
(assert (= (state-type |47|) |IoT Device Zone|))
(assert (= ((as const (Array asset-state-relation-sort Bool)) false)
   asset-state-relation))
(assert (let ((a!1 (store (store (store ((as const (Array contains-relation-sort Bool))
                                  false)
                                (contains-relation-sort |47| |2|)
                                true)
                         (contains-relation-sort |47| |4|)
                         true)
                  (contains-relation-sort |47| |6|)
                  true)))
  (= (store (store a!1 (contains-relation-sort |47| |10|) true)
            (contains-relation-sort |47| |46|)
            true)
     contains-relation)))
(assert (= (transition-type |1|) |Wireless Connector|))
(assert (and (= (source |1|) |2|) (= (target |1|) |6|)))
(assert (or (= (trans-attr |1| Authentication) undefined)
    (= (trans-attr |1| Authentication) strong)
    (= (trans-attr |1| Authentication) Yes)
    (= (trans-attr |1| Authentication) No)
    (= (trans-attr |1| Authentication) undefined)
    (= (trans-attr |1| Authentication) strong)
    (= (trans-attr |1| Authentication) Yes)
    (= (trans-attr |1| Authentication) No)
    (= (trans-attr |1| Authentication) undefined)
    (= (trans-attr |1| Authentication) strong)
    (= (trans-attr |1| Authentication) Yes)
    (= (trans-attr |1| Authentication) No)))
(assert (or (= (trans-attr |1| |Credential Asset|) undefined)
    (= (trans-attr |1| |Credential Asset|) Yes)
    (= (trans-attr |1| |Credential Asset|) No)
    (= (trans-attr |1| |Credential Asset|) encrypted)
    (= (trans-attr |1| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |1| |Credential Asset|) undefined)
    (= (trans-attr |1| |Credential Asset|) Yes)
    (= (trans-attr |1| |Credential Asset|) No)
    (= (trans-attr |1| |Credential Asset|) encrypted)
    (= (trans-attr |1| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |1| |Credential Asset|) undefined)
    (= (trans-attr |1| |Credential Asset|) Yes)
    (= (trans-attr |1| |Credential Asset|) No)
    (= (trans-attr |1| |Credential Asset|) encrypted)
    (= (trans-attr |1| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |1| Encrypted) undefined)
    (= (trans-attr |1| Encrypted) Yes)
    (= (trans-attr |1| Encrypted) No)
    (= (trans-attr |1| Encrypted) strong)
    (= (trans-attr |1| Encrypted) undefined)
    (= (trans-attr |1| Encrypted) Yes)
    (= (trans-attr |1| Encrypted) No)
    (= (trans-attr |1| Encrypted) strong)
    (= (trans-attr |1| Encrypted) undefined)
    (= (trans-attr |1| Encrypted) Yes)
    (= (trans-attr |1| Encrypted) No)
    (= (trans-attr |1| Encrypted) strong)))
(assert (or (= (trans-attr |1| |Encryption Method|) undefined)
    (= (trans-attr |1| |Encryption Method|) strong)
    (= (trans-attr |1| |Encryption Method|) weak)
    (= (trans-attr |1| |Encryption Method|) undefined)
    (= (trans-attr |1| |Encryption Method|) strong)
    (= (trans-attr |1| |Encryption Method|) weak)
    (= (trans-attr |1| |Encryption Method|) undefined)
    (= (trans-attr |1| |Encryption Method|) strong)
    (= (trans-attr |1| |Encryption Method|) weak)))
(assert (= (trans-attr |1| |Access Control|) missing))
(assert (= (trans-attr |1| |Activity Logging|) missing))
(assert (= (trans-attr |1| Administration) missing))
(assert (= (trans-attr |1| |Allows User Input|) missing))
(assert (= (trans-attr |1| |Anomaly Detection|) missing))
(assert (= (trans-attr |1| |API Type|) missing))
(assert (= (trans-attr |1| |Approved License|) missing))
(assert (= (trans-attr |1| Auditing) missing))
(assert (= (trans-attr |1| Authorization) missing))
(assert (= (trans-attr |1| Availability) missing))
(assert (= (trans-attr |1| Bandwidth) missing))
(assert (= (trans-attr |1| |Certificate Checks|) missing))
(assert (= (trans-attr |1| |Coding guideline|) missing))
(assert (= (trans-attr |1| |Communication Latency|) missing))
(assert (= (trans-attr |1| |Communication Reliability|) missing))
(assert (= (trans-attr |1| Confidentiality) missing))
(assert (= (trans-attr |1| Content) missing))
(assert (= (trans-attr |1| |Counterfeit Detection|) missing))
(assert (= (trans-attr |1| Criticality) missing))
(assert (= (trans-attr |1| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |1| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |1| |Data Backup|) missing))
(assert (= (trans-attr |1| |Data safety integrity|) missing))
(assert (= (trans-attr |1| |Data security integrity|) missing))
(assert (= (trans-attr |1| |Data Store|) missing))
(assert (= (trans-attr |1| |DDoS Mitigation|) missing))
(assert (= (trans-attr |1| |Device Fingerprint|) missing))
(assert (= (trans-attr |1| |Digital Signature|) missing))
(assert (= (trans-attr |1| Encryption) missing))
(assert (= (trans-attr |1| |Encryption Time|) missing))
(assert (= (trans-attr |1| |Error Rate|) missing))
(assert (= (trans-attr |1| Feedback) missing))
(assert (= (trans-attr |1| |Financial Asset|) missing))
(assert (= (trans-attr |1| Firmware) missing))
(assert (= (trans-attr |1| |Input Sanitization|) missing))
(assert (= (trans-attr |1| |Input Validation|) missing))
(assert (= (trans-attr |1| Integrity) missing))
(assert (= (trans-attr |1| |Key Length|) missing))
(assert (= (trans-attr |1| |Key Revocation|) missing))
(assert (= (trans-attr |1| Language) missing))
(assert (= (trans-attr |1| License) missing))
(assert (= (trans-attr |1| Location) missing))
(assert (= (trans-attr |1| |Malware Protection|) missing))
(assert (= (trans-attr |1| Managed) missing))
(assert (= (trans-attr |1| |Maximum Value|) missing))
(assert (= (trans-attr |1| |Memory Type|) missing))
(assert (= (trans-attr |1| |Minimum Value|) missing))
(assert (= (trans-attr |1| |Network Technology|) missing))
(assert (= (trans-attr |1| |Operating system|) missing))
(assert (= (trans-attr |1| |Operational Criticality|) missing))
(assert (= (trans-attr |1| Permissions) missing))
(assert (= (trans-attr |1| |Physical Location|) missing))
(assert (= (trans-attr |1| |Power consumption|) missing))
(assert (= (trans-attr |1| |Privacy Asset|) missing))
(assert (= (trans-attr |1| |Processing Time|) missing))
(assert (= (trans-attr |1| |Protected Execution Environment|) missing))
(assert (= (trans-attr |1| |Protocol version|) missing))
(assert (= (trans-attr |1| Protocols) missing))
(assert (= (trans-attr |1| |PtwoP Capability|) missing))
(assert (= (trans-attr |1| Range) missing))
(assert (= (trans-attr |1| Redundancy) missing))
(assert (= (trans-attr |1| |Reset capabilities|) missing))
(assert (= (trans-attr |1| Roles) missing))
(assert (= (trans-attr |1| |Secure Boot|) missing))
(assert (= (trans-attr |1| |Secure Session Handling|) missing))
(assert (= (trans-attr |1| |Secure Storage|) missing))
(assert (= (trans-attr |1| |Secure Update|) missing))
(assert (= (trans-attr |1| |Sensor measurement type|) missing))
(assert (= (trans-attr |1| |Shared resources|) missing))
(assert (= (trans-attr |1| Software) missing))
(assert (= (trans-attr |1| |Software APIs|) missing))
(assert (= (trans-attr |1| |Standard Password|) missing))
(assert (= (trans-attr |1| Storage) missing))
(assert (= (trans-attr |1| |Tamper Protection|) missing))
(assert (= (trans-attr |1| |Token Signing|) missing))
(assert (= (trans-attr |1| |Token Validation|) missing))
(assert (= (trans-attr |1| Troughput) missing))
(assert (= (trans-attr |1| Unit) missing))
(assert (= (trans-attr |1| |Update capabilities|) missing))
(assert (= (trans-attr |1| Updates) missing))
(assert (= (trans-attr |1| |URL Blacklisting|) missing))
(assert (= (trans-attr |1| |User File Upload|) missing))
(assert (= (trans-attr |1| |User Interfaces|) missing))
(assert (= (trans-attr |1| |User Management|) missing))
(assert (= (trans-attr |1| |Wired interface|) missing))
(assert (= (trans-attr |1| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |1| |Wireless Interface|) missing))
(assert (= (transition-type |2|) |Wireless Connector|))
(assert (and (= (source |2|) |4|) (= (target |2|) |6|)))
(assert (or (= (trans-attr |2| Authentication) undefined)
    (= (trans-attr |2| Authentication) strong)
    (= (trans-attr |2| Authentication) Yes)
    (= (trans-attr |2| Authentication) No)
    (= (trans-attr |2| Authentication) undefined)
    (= (trans-attr |2| Authentication) strong)
    (= (trans-attr |2| Authentication) Yes)
    (= (trans-attr |2| Authentication) No)
    (= (trans-attr |2| Authentication) undefined)
    (= (trans-attr |2| Authentication) strong)
    (= (trans-attr |2| Authentication) Yes)
    (= (trans-attr |2| Authentication) No)))
(assert (or (= (trans-attr |2| |Credential Asset|) undefined)
    (= (trans-attr |2| |Credential Asset|) Yes)
    (= (trans-attr |2| |Credential Asset|) No)
    (= (trans-attr |2| |Credential Asset|) encrypted)
    (= (trans-attr |2| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |2| |Credential Asset|) undefined)
    (= (trans-attr |2| |Credential Asset|) Yes)
    (= (trans-attr |2| |Credential Asset|) No)
    (= (trans-attr |2| |Credential Asset|) encrypted)
    (= (trans-attr |2| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |2| |Credential Asset|) undefined)
    (= (trans-attr |2| |Credential Asset|) Yes)
    (= (trans-attr |2| |Credential Asset|) No)
    (= (trans-attr |2| |Credential Asset|) encrypted)
    (= (trans-attr |2| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |2| Encrypted) undefined)
    (= (trans-attr |2| Encrypted) Yes)
    (= (trans-attr |2| Encrypted) No)
    (= (trans-attr |2| Encrypted) strong)
    (= (trans-attr |2| Encrypted) undefined)
    (= (trans-attr |2| Encrypted) Yes)
    (= (trans-attr |2| Encrypted) No)
    (= (trans-attr |2| Encrypted) strong)
    (= (trans-attr |2| Encrypted) undefined)
    (= (trans-attr |2| Encrypted) Yes)
    (= (trans-attr |2| Encrypted) No)
    (= (trans-attr |2| Encrypted) strong)))
(assert (or (= (trans-attr |2| |Encryption Method|) undefined)
    (= (trans-attr |2| |Encryption Method|) strong)
    (= (trans-attr |2| |Encryption Method|) weak)
    (= (trans-attr |2| |Encryption Method|) undefined)
    (= (trans-attr |2| |Encryption Method|) strong)
    (= (trans-attr |2| |Encryption Method|) weak)
    (= (trans-attr |2| |Encryption Method|) undefined)
    (= (trans-attr |2| |Encryption Method|) strong)
    (= (trans-attr |2| |Encryption Method|) weak)))
(assert (= (trans-attr |2| |Access Control|) missing))
(assert (= (trans-attr |2| |Activity Logging|) missing))
(assert (= (trans-attr |2| Administration) missing))
(assert (= (trans-attr |2| |Allows User Input|) missing))
(assert (= (trans-attr |2| |Anomaly Detection|) missing))
(assert (= (trans-attr |2| |API Type|) missing))
(assert (= (trans-attr |2| |Approved License|) missing))
(assert (= (trans-attr |2| Auditing) missing))
(assert (= (trans-attr |2| Authorization) missing))
(assert (= (trans-attr |2| Availability) missing))
(assert (= (trans-attr |2| Bandwidth) missing))
(assert (= (trans-attr |2| |Certificate Checks|) missing))
(assert (= (trans-attr |2| |Coding guideline|) missing))
(assert (= (trans-attr |2| |Communication Latency|) missing))
(assert (= (trans-attr |2| |Communication Reliability|) missing))
(assert (= (trans-attr |2| Confidentiality) missing))
(assert (= (trans-attr |2| Content) missing))
(assert (= (trans-attr |2| |Counterfeit Detection|) missing))
(assert (= (trans-attr |2| Criticality) missing))
(assert (= (trans-attr |2| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |2| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |2| |Data Backup|) missing))
(assert (= (trans-attr |2| |Data safety integrity|) missing))
(assert (= (trans-attr |2| |Data security integrity|) missing))
(assert (= (trans-attr |2| |Data Store|) missing))
(assert (= (trans-attr |2| |DDoS Mitigation|) missing))
(assert (= (trans-attr |2| |Device Fingerprint|) missing))
(assert (= (trans-attr |2| |Digital Signature|) missing))
(assert (= (trans-attr |2| Encryption) missing))
(assert (= (trans-attr |2| |Encryption Time|) missing))
(assert (= (trans-attr |2| |Error Rate|) missing))
(assert (= (trans-attr |2| Feedback) missing))
(assert (= (trans-attr |2| |Financial Asset|) missing))
(assert (= (trans-attr |2| Firmware) missing))
(assert (= (trans-attr |2| |Input Sanitization|) missing))
(assert (= (trans-attr |2| |Input Validation|) missing))
(assert (= (trans-attr |2| Integrity) missing))
(assert (= (trans-attr |2| |Key Length|) missing))
(assert (= (trans-attr |2| |Key Revocation|) missing))
(assert (= (trans-attr |2| Language) missing))
(assert (= (trans-attr |2| License) missing))
(assert (= (trans-attr |2| Location) missing))
(assert (= (trans-attr |2| |Malware Protection|) missing))
(assert (= (trans-attr |2| Managed) missing))
(assert (= (trans-attr |2| |Maximum Value|) missing))
(assert (= (trans-attr |2| |Memory Type|) missing))
(assert (= (trans-attr |2| |Minimum Value|) missing))
(assert (= (trans-attr |2| |Network Technology|) missing))
(assert (= (trans-attr |2| |Operating system|) missing))
(assert (= (trans-attr |2| |Operational Criticality|) missing))
(assert (= (trans-attr |2| Permissions) missing))
(assert (= (trans-attr |2| |Physical Location|) missing))
(assert (= (trans-attr |2| |Power consumption|) missing))
(assert (= (trans-attr |2| |Privacy Asset|) missing))
(assert (= (trans-attr |2| |Processing Time|) missing))
(assert (= (trans-attr |2| |Protected Execution Environment|) missing))
(assert (= (trans-attr |2| |Protocol version|) missing))
(assert (= (trans-attr |2| Protocols) missing))
(assert (= (trans-attr |2| |PtwoP Capability|) missing))
(assert (= (trans-attr |2| Range) missing))
(assert (= (trans-attr |2| Redundancy) missing))
(assert (= (trans-attr |2| |Reset capabilities|) missing))
(assert (= (trans-attr |2| Roles) missing))
(assert (= (trans-attr |2| |Secure Boot|) missing))
(assert (= (trans-attr |2| |Secure Session Handling|) missing))
(assert (= (trans-attr |2| |Secure Storage|) missing))
(assert (= (trans-attr |2| |Secure Update|) missing))
(assert (= (trans-attr |2| |Sensor measurement type|) missing))
(assert (= (trans-attr |2| |Shared resources|) missing))
(assert (= (trans-attr |2| Software) missing))
(assert (= (trans-attr |2| |Software APIs|) missing))
(assert (= (trans-attr |2| |Standard Password|) missing))
(assert (= (trans-attr |2| Storage) missing))
(assert (= (trans-attr |2| |Tamper Protection|) missing))
(assert (= (trans-attr |2| |Token Signing|) missing))
(assert (= (trans-attr |2| |Token Validation|) missing))
(assert (= (trans-attr |2| Troughput) missing))
(assert (= (trans-attr |2| Unit) missing))
(assert (= (trans-attr |2| |Update capabilities|) missing))
(assert (= (trans-attr |2| Updates) missing))
(assert (= (trans-attr |2| |URL Blacklisting|) missing))
(assert (= (trans-attr |2| |User File Upload|) missing))
(assert (= (trans-attr |2| |User Interfaces|) missing))
(assert (= (trans-attr |2| |User Management|) missing))
(assert (= (trans-attr |2| |Wired interface|) missing))
(assert (= (trans-attr |2| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |2| |Wireless Interface|) missing))
(assert (= (transition-type |10|) |Wireless Connector|))
(assert (and (= (source |10|) |10|) (= (target |10|) |6|)))
(assert (or (= (trans-attr |10| Authentication) undefined)
    (= (trans-attr |10| Authentication) strong)
    (= (trans-attr |10| Authentication) Yes)
    (= (trans-attr |10| Authentication) No)
    (= (trans-attr |10| Authentication) undefined)
    (= (trans-attr |10| Authentication) strong)
    (= (trans-attr |10| Authentication) Yes)
    (= (trans-attr |10| Authentication) No)
    (= (trans-attr |10| Authentication) undefined)
    (= (trans-attr |10| Authentication) strong)
    (= (trans-attr |10| Authentication) Yes)
    (= (trans-attr |10| Authentication) No)))
(assert (or (= (trans-attr |10| |Credential Asset|) undefined)
    (= (trans-attr |10| |Credential Asset|) Yes)
    (= (trans-attr |10| |Credential Asset|) No)
    (= (trans-attr |10| |Credential Asset|) encrypted)
    (= (trans-attr |10| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |10| |Credential Asset|) undefined)
    (= (trans-attr |10| |Credential Asset|) Yes)
    (= (trans-attr |10| |Credential Asset|) No)
    (= (trans-attr |10| |Credential Asset|) encrypted)
    (= (trans-attr |10| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |10| |Credential Asset|) undefined)
    (= (trans-attr |10| |Credential Asset|) Yes)
    (= (trans-attr |10| |Credential Asset|) No)
    (= (trans-attr |10| |Credential Asset|) encrypted)
    (= (trans-attr |10| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |10| Encrypted) undefined)
    (= (trans-attr |10| Encrypted) Yes)
    (= (trans-attr |10| Encrypted) No)
    (= (trans-attr |10| Encrypted) strong)
    (= (trans-attr |10| Encrypted) undefined)
    (= (trans-attr |10| Encrypted) Yes)
    (= (trans-attr |10| Encrypted) No)
    (= (trans-attr |10| Encrypted) strong)
    (= (trans-attr |10| Encrypted) undefined)
    (= (trans-attr |10| Encrypted) Yes)
    (= (trans-attr |10| Encrypted) No)
    (= (trans-attr |10| Encrypted) strong)))
(assert (or (= (trans-attr |10| |Encryption Method|) undefined)
    (= (trans-attr |10| |Encryption Method|) strong)
    (= (trans-attr |10| |Encryption Method|) weak)
    (= (trans-attr |10| |Encryption Method|) undefined)
    (= (trans-attr |10| |Encryption Method|) strong)
    (= (trans-attr |10| |Encryption Method|) weak)
    (= (trans-attr |10| |Encryption Method|) undefined)
    (= (trans-attr |10| |Encryption Method|) strong)
    (= (trans-attr |10| |Encryption Method|) weak)))
(assert (= (trans-attr |10| |Access Control|) missing))
(assert (= (trans-attr |10| |Activity Logging|) missing))
(assert (= (trans-attr |10| Administration) missing))
(assert (= (trans-attr |10| |Allows User Input|) missing))
(assert (= (trans-attr |10| |Anomaly Detection|) missing))
(assert (= (trans-attr |10| |API Type|) missing))
(assert (= (trans-attr |10| |Approved License|) missing))
(assert (= (trans-attr |10| Auditing) missing))
(assert (= (trans-attr |10| Authorization) missing))
(assert (= (trans-attr |10| Availability) missing))
(assert (= (trans-attr |10| Bandwidth) missing))
(assert (= (trans-attr |10| |Certificate Checks|) missing))
(assert (= (trans-attr |10| |Coding guideline|) missing))
(assert (= (trans-attr |10| |Communication Latency|) missing))
(assert (= (trans-attr |10| |Communication Reliability|) missing))
(assert (= (trans-attr |10| Confidentiality) missing))
(assert (= (trans-attr |10| Content) missing))
(assert (= (trans-attr |10| |Counterfeit Detection|) missing))
(assert (= (trans-attr |10| Criticality) missing))
(assert (= (trans-attr |10| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |10| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |10| |Data Backup|) missing))
(assert (= (trans-attr |10| |Data safety integrity|) missing))
(assert (= (trans-attr |10| |Data security integrity|) missing))
(assert (= (trans-attr |10| |Data Store|) missing))
(assert (= (trans-attr |10| |DDoS Mitigation|) missing))
(assert (= (trans-attr |10| |Device Fingerprint|) missing))
(assert (= (trans-attr |10| |Digital Signature|) missing))
(assert (= (trans-attr |10| Encryption) missing))
(assert (= (trans-attr |10| |Encryption Time|) missing))
(assert (= (trans-attr |10| |Error Rate|) missing))
(assert (= (trans-attr |10| Feedback) missing))
(assert (= (trans-attr |10| |Financial Asset|) missing))
(assert (= (trans-attr |10| Firmware) missing))
(assert (= (trans-attr |10| |Input Sanitization|) missing))
(assert (= (trans-attr |10| |Input Validation|) missing))
(assert (= (trans-attr |10| Integrity) missing))
(assert (= (trans-attr |10| |Key Length|) missing))
(assert (= (trans-attr |10| |Key Revocation|) missing))
(assert (= (trans-attr |10| Language) missing))
(assert (= (trans-attr |10| License) missing))
(assert (= (trans-attr |10| Location) missing))
(assert (= (trans-attr |10| |Malware Protection|) missing))
(assert (= (trans-attr |10| Managed) missing))
(assert (= (trans-attr |10| |Maximum Value|) missing))
(assert (= (trans-attr |10| |Memory Type|) missing))
(assert (= (trans-attr |10| |Minimum Value|) missing))
(assert (= (trans-attr |10| |Network Technology|) missing))
(assert (= (trans-attr |10| |Operating system|) missing))
(assert (= (trans-attr |10| |Operational Criticality|) missing))
(assert (= (trans-attr |10| Permissions) missing))
(assert (= (trans-attr |10| |Physical Location|) missing))
(assert (= (trans-attr |10| |Power consumption|) missing))
(assert (= (trans-attr |10| |Privacy Asset|) missing))
(assert (= (trans-attr |10| |Processing Time|) missing))
(assert (= (trans-attr |10| |Protected Execution Environment|) missing))
(assert (= (trans-attr |10| |Protocol version|) missing))
(assert (= (trans-attr |10| Protocols) missing))
(assert (= (trans-attr |10| |PtwoP Capability|) missing))
(assert (= (trans-attr |10| Range) missing))
(assert (= (trans-attr |10| Redundancy) missing))
(assert (= (trans-attr |10| |Reset capabilities|) missing))
(assert (= (trans-attr |10| Roles) missing))
(assert (= (trans-attr |10| |Secure Boot|) missing))
(assert (= (trans-attr |10| |Secure Session Handling|) missing))
(assert (= (trans-attr |10| |Secure Storage|) missing))
(assert (= (trans-attr |10| |Secure Update|) missing))
(assert (= (trans-attr |10| |Sensor measurement type|) missing))
(assert (= (trans-attr |10| |Shared resources|) missing))
(assert (= (trans-attr |10| Software) missing))
(assert (= (trans-attr |10| |Software APIs|) missing))
(assert (= (trans-attr |10| |Standard Password|) missing))
(assert (= (trans-attr |10| Storage) missing))
(assert (= (trans-attr |10| |Tamper Protection|) missing))
(assert (= (trans-attr |10| |Token Signing|) missing))
(assert (= (trans-attr |10| |Token Validation|) missing))
(assert (= (trans-attr |10| Troughput) missing))
(assert (= (trans-attr |10| Unit) missing))
(assert (= (trans-attr |10| |Update capabilities|) missing))
(assert (= (trans-attr |10| Updates) missing))
(assert (= (trans-attr |10| |URL Blacklisting|) missing))
(assert (= (trans-attr |10| |User File Upload|) missing))
(assert (= (trans-attr |10| |User Interfaces|) missing))
(assert (= (trans-attr |10| |User Management|) missing))
(assert (= (trans-attr |10| |Wired interface|) missing))
(assert (= (trans-attr |10| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |10| |Wireless Interface|) missing))
(assert (= (transition-type |11|) |Wireless Connector|))
(assert (and (= (source |11|) |6|) (= (target |11|) |10|)))
(assert (or (= (trans-attr |11| Authentication) undefined)
    (= (trans-attr |11| Authentication) strong)
    (= (trans-attr |11| Authentication) Yes)
    (= (trans-attr |11| Authentication) No)
    (= (trans-attr |11| Authentication) undefined)
    (= (trans-attr |11| Authentication) strong)
    (= (trans-attr |11| Authentication) Yes)
    (= (trans-attr |11| Authentication) No)
    (= (trans-attr |11| Authentication) undefined)
    (= (trans-attr |11| Authentication) strong)
    (= (trans-attr |11| Authentication) Yes)
    (= (trans-attr |11| Authentication) No)))
(assert (or (= (trans-attr |11| |Credential Asset|) undefined)
    (= (trans-attr |11| |Credential Asset|) Yes)
    (= (trans-attr |11| |Credential Asset|) No)
    (= (trans-attr |11| |Credential Asset|) encrypted)
    (= (trans-attr |11| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |11| |Credential Asset|) undefined)
    (= (trans-attr |11| |Credential Asset|) Yes)
    (= (trans-attr |11| |Credential Asset|) No)
    (= (trans-attr |11| |Credential Asset|) encrypted)
    (= (trans-attr |11| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |11| |Credential Asset|) undefined)
    (= (trans-attr |11| |Credential Asset|) Yes)
    (= (trans-attr |11| |Credential Asset|) No)
    (= (trans-attr |11| |Credential Asset|) encrypted)
    (= (trans-attr |11| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |11| Encrypted) undefined)
    (= (trans-attr |11| Encrypted) Yes)
    (= (trans-attr |11| Encrypted) No)
    (= (trans-attr |11| Encrypted) strong)
    (= (trans-attr |11| Encrypted) undefined)
    (= (trans-attr |11| Encrypted) Yes)
    (= (trans-attr |11| Encrypted) No)
    (= (trans-attr |11| Encrypted) strong)
    (= (trans-attr |11| Encrypted) undefined)
    (= (trans-attr |11| Encrypted) Yes)
    (= (trans-attr |11| Encrypted) No)
    (= (trans-attr |11| Encrypted) strong)))
(assert (or (= (trans-attr |11| |Encryption Method|) undefined)
    (= (trans-attr |11| |Encryption Method|) strong)
    (= (trans-attr |11| |Encryption Method|) weak)
    (= (trans-attr |11| |Encryption Method|) undefined)
    (= (trans-attr |11| |Encryption Method|) strong)
    (= (trans-attr |11| |Encryption Method|) weak)
    (= (trans-attr |11| |Encryption Method|) undefined)
    (= (trans-attr |11| |Encryption Method|) strong)
    (= (trans-attr |11| |Encryption Method|) weak)))
(assert (= (trans-attr |11| |Access Control|) missing))
(assert (= (trans-attr |11| |Activity Logging|) missing))
(assert (= (trans-attr |11| Administration) missing))
(assert (= (trans-attr |11| |Allows User Input|) missing))
(assert (= (trans-attr |11| |Anomaly Detection|) missing))
(assert (= (trans-attr |11| |API Type|) missing))
(assert (= (trans-attr |11| |Approved License|) missing))
(assert (= (trans-attr |11| Auditing) missing))
(assert (= (trans-attr |11| Authorization) missing))
(assert (= (trans-attr |11| Availability) missing))
(assert (= (trans-attr |11| Bandwidth) missing))
(assert (= (trans-attr |11| |Certificate Checks|) missing))
(assert (= (trans-attr |11| |Coding guideline|) missing))
(assert (= (trans-attr |11| |Communication Latency|) missing))
(assert (= (trans-attr |11| |Communication Reliability|) missing))
(assert (= (trans-attr |11| Confidentiality) missing))
(assert (= (trans-attr |11| Content) missing))
(assert (= (trans-attr |11| |Counterfeit Detection|) missing))
(assert (= (trans-attr |11| Criticality) missing))
(assert (= (trans-attr |11| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |11| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |11| |Data Backup|) missing))
(assert (= (trans-attr |11| |Data safety integrity|) missing))
(assert (= (trans-attr |11| |Data security integrity|) missing))
(assert (= (trans-attr |11| |Data Store|) missing))
(assert (= (trans-attr |11| |DDoS Mitigation|) missing))
(assert (= (trans-attr |11| |Device Fingerprint|) missing))
(assert (= (trans-attr |11| |Digital Signature|) missing))
(assert (= (trans-attr |11| Encryption) missing))
(assert (= (trans-attr |11| |Encryption Time|) missing))
(assert (= (trans-attr |11| |Error Rate|) missing))
(assert (= (trans-attr |11| Feedback) missing))
(assert (= (trans-attr |11| |Financial Asset|) missing))
(assert (= (trans-attr |11| Firmware) missing))
(assert (= (trans-attr |11| |Input Sanitization|) missing))
(assert (= (trans-attr |11| |Input Validation|) missing))
(assert (= (trans-attr |11| Integrity) missing))
(assert (= (trans-attr |11| |Key Length|) missing))
(assert (= (trans-attr |11| |Key Revocation|) missing))
(assert (= (trans-attr |11| Language) missing))
(assert (= (trans-attr |11| License) missing))
(assert (= (trans-attr |11| Location) missing))
(assert (= (trans-attr |11| |Malware Protection|) missing))
(assert (= (trans-attr |11| Managed) missing))
(assert (= (trans-attr |11| |Maximum Value|) missing))
(assert (= (trans-attr |11| |Memory Type|) missing))
(assert (= (trans-attr |11| |Minimum Value|) missing))
(assert (= (trans-attr |11| |Network Technology|) missing))
(assert (= (trans-attr |11| |Operating system|) missing))
(assert (= (trans-attr |11| |Operational Criticality|) missing))
(assert (= (trans-attr |11| Permissions) missing))
(assert (= (trans-attr |11| |Physical Location|) missing))
(assert (= (trans-attr |11| |Power consumption|) missing))
(assert (= (trans-attr |11| |Privacy Asset|) missing))
(assert (= (trans-attr |11| |Processing Time|) missing))
(assert (= (trans-attr |11| |Protected Execution Environment|) missing))
(assert (= (trans-attr |11| |Protocol version|) missing))
(assert (= (trans-attr |11| Protocols) missing))
(assert (= (trans-attr |11| |PtwoP Capability|) missing))
(assert (= (trans-attr |11| Range) missing))
(assert (= (trans-attr |11| Redundancy) missing))
(assert (= (trans-attr |11| |Reset capabilities|) missing))
(assert (= (trans-attr |11| Roles) missing))
(assert (= (trans-attr |11| |Secure Boot|) missing))
(assert (= (trans-attr |11| |Secure Session Handling|) missing))
(assert (= (trans-attr |11| |Secure Storage|) missing))
(assert (= (trans-attr |11| |Secure Update|) missing))
(assert (= (trans-attr |11| |Sensor measurement type|) missing))
(assert (= (trans-attr |11| |Shared resources|) missing))
(assert (= (trans-attr |11| Software) missing))
(assert (= (trans-attr |11| |Software APIs|) missing))
(assert (= (trans-attr |11| |Standard Password|) missing))
(assert (= (trans-attr |11| Storage) missing))
(assert (= (trans-attr |11| |Tamper Protection|) missing))
(assert (= (trans-attr |11| |Token Signing|) missing))
(assert (= (trans-attr |11| |Token Validation|) missing))
(assert (= (trans-attr |11| Troughput) missing))
(assert (= (trans-attr |11| Unit) missing))
(assert (= (trans-attr |11| |Update capabilities|) missing))
(assert (= (trans-attr |11| Updates) missing))
(assert (= (trans-attr |11| |URL Blacklisting|) missing))
(assert (= (trans-attr |11| |User File Upload|) missing))
(assert (= (trans-attr |11| |User Interfaces|) missing))
(assert (= (trans-attr |11| |User Management|) missing))
(assert (= (trans-attr |11| |Wired interface|) missing))
(assert (= (trans-attr |11| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |11| |Wireless Interface|) missing))
(assert (= (transition-type |13|) |Wireless Connector|))
(assert (and (= (source |13|) |12|) (= (target |13|) |3|)))
(assert (or (= (trans-attr |13| Authentication) undefined)
    (= (trans-attr |13| Authentication) strong)
    (= (trans-attr |13| Authentication) Yes)
    (= (trans-attr |13| Authentication) No)
    (= (trans-attr |13| Authentication) undefined)
    (= (trans-attr |13| Authentication) strong)
    (= (trans-attr |13| Authentication) Yes)
    (= (trans-attr |13| Authentication) No)
    (= (trans-attr |13| Authentication) undefined)
    (= (trans-attr |13| Authentication) strong)
    (= (trans-attr |13| Authentication) Yes)
    (= (trans-attr |13| Authentication) No)))
(assert (or (= (trans-attr |13| |Credential Asset|) undefined)
    (= (trans-attr |13| |Credential Asset|) Yes)
    (= (trans-attr |13| |Credential Asset|) No)
    (= (trans-attr |13| |Credential Asset|) encrypted)
    (= (trans-attr |13| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |13| |Credential Asset|) undefined)
    (= (trans-attr |13| |Credential Asset|) Yes)
    (= (trans-attr |13| |Credential Asset|) No)
    (= (trans-attr |13| |Credential Asset|) encrypted)
    (= (trans-attr |13| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |13| |Credential Asset|) undefined)
    (= (trans-attr |13| |Credential Asset|) Yes)
    (= (trans-attr |13| |Credential Asset|) No)
    (= (trans-attr |13| |Credential Asset|) encrypted)
    (= (trans-attr |13| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |13| Encrypted) undefined)
    (= (trans-attr |13| Encrypted) Yes)
    (= (trans-attr |13| Encrypted) No)
    (= (trans-attr |13| Encrypted) strong)
    (= (trans-attr |13| Encrypted) undefined)
    (= (trans-attr |13| Encrypted) Yes)
    (= (trans-attr |13| Encrypted) No)
    (= (trans-attr |13| Encrypted) strong)
    (= (trans-attr |13| Encrypted) undefined)
    (= (trans-attr |13| Encrypted) Yes)
    (= (trans-attr |13| Encrypted) No)
    (= (trans-attr |13| Encrypted) strong)))
(assert (or (= (trans-attr |13| |Encryption Method|) undefined)
    (= (trans-attr |13| |Encryption Method|) strong)
    (= (trans-attr |13| |Encryption Method|) weak)
    (= (trans-attr |13| |Encryption Method|) undefined)
    (= (trans-attr |13| |Encryption Method|) strong)
    (= (trans-attr |13| |Encryption Method|) weak)
    (= (trans-attr |13| |Encryption Method|) undefined)
    (= (trans-attr |13| |Encryption Method|) strong)
    (= (trans-attr |13| |Encryption Method|) weak)))
(assert (= (trans-attr |13| |Access Control|) missing))
(assert (= (trans-attr |13| |Activity Logging|) missing))
(assert (= (trans-attr |13| Administration) missing))
(assert (= (trans-attr |13| |Allows User Input|) missing))
(assert (= (trans-attr |13| |Anomaly Detection|) missing))
(assert (= (trans-attr |13| |API Type|) missing))
(assert (= (trans-attr |13| |Approved License|) missing))
(assert (= (trans-attr |13| Auditing) missing))
(assert (= (trans-attr |13| Authorization) missing))
(assert (= (trans-attr |13| Availability) missing))
(assert (= (trans-attr |13| Bandwidth) missing))
(assert (= (trans-attr |13| |Certificate Checks|) missing))
(assert (= (trans-attr |13| |Coding guideline|) missing))
(assert (= (trans-attr |13| |Communication Latency|) missing))
(assert (= (trans-attr |13| |Communication Reliability|) missing))
(assert (= (trans-attr |13| Confidentiality) missing))
(assert (= (trans-attr |13| Content) missing))
(assert (= (trans-attr |13| |Counterfeit Detection|) missing))
(assert (= (trans-attr |13| Criticality) missing))
(assert (= (trans-attr |13| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |13| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |13| |Data Backup|) missing))
(assert (= (trans-attr |13| |Data safety integrity|) missing))
(assert (= (trans-attr |13| |Data security integrity|) missing))
(assert (= (trans-attr |13| |Data Store|) missing))
(assert (= (trans-attr |13| |DDoS Mitigation|) missing))
(assert (= (trans-attr |13| |Device Fingerprint|) missing))
(assert (= (trans-attr |13| |Digital Signature|) missing))
(assert (= (trans-attr |13| Encryption) missing))
(assert (= (trans-attr |13| |Encryption Time|) missing))
(assert (= (trans-attr |13| |Error Rate|) missing))
(assert (= (trans-attr |13| Feedback) missing))
(assert (= (trans-attr |13| |Financial Asset|) missing))
(assert (= (trans-attr |13| Firmware) missing))
(assert (= (trans-attr |13| |Input Sanitization|) missing))
(assert (= (trans-attr |13| |Input Validation|) missing))
(assert (= (trans-attr |13| Integrity) missing))
(assert (= (trans-attr |13| |Key Length|) missing))
(assert (= (trans-attr |13| |Key Revocation|) missing))
(assert (= (trans-attr |13| Language) missing))
(assert (= (trans-attr |13| License) missing))
(assert (= (trans-attr |13| Location) missing))
(assert (= (trans-attr |13| |Malware Protection|) missing))
(assert (= (trans-attr |13| Managed) missing))
(assert (= (trans-attr |13| |Maximum Value|) missing))
(assert (= (trans-attr |13| |Memory Type|) missing))
(assert (= (trans-attr |13| |Minimum Value|) missing))
(assert (= (trans-attr |13| |Network Technology|) missing))
(assert (= (trans-attr |13| |Operating system|) missing))
(assert (= (trans-attr |13| |Operational Criticality|) missing))
(assert (= (trans-attr |13| Permissions) missing))
(assert (= (trans-attr |13| |Physical Location|) missing))
(assert (= (trans-attr |13| |Power consumption|) missing))
(assert (= (trans-attr |13| |Privacy Asset|) missing))
(assert (= (trans-attr |13| |Processing Time|) missing))
(assert (= (trans-attr |13| |Protected Execution Environment|) missing))
(assert (= (trans-attr |13| |Protocol version|) missing))
(assert (= (trans-attr |13| Protocols) missing))
(assert (= (trans-attr |13| |PtwoP Capability|) missing))
(assert (= (trans-attr |13| Range) missing))
(assert (= (trans-attr |13| Redundancy) missing))
(assert (= (trans-attr |13| |Reset capabilities|) missing))
(assert (= (trans-attr |13| Roles) missing))
(assert (= (trans-attr |13| |Secure Boot|) missing))
(assert (= (trans-attr |13| |Secure Session Handling|) missing))
(assert (= (trans-attr |13| |Secure Storage|) missing))
(assert (= (trans-attr |13| |Secure Update|) missing))
(assert (= (trans-attr |13| |Sensor measurement type|) missing))
(assert (= (trans-attr |13| |Shared resources|) missing))
(assert (= (trans-attr |13| Software) missing))
(assert (= (trans-attr |13| |Software APIs|) missing))
(assert (= (trans-attr |13| |Standard Password|) missing))
(assert (= (trans-attr |13| Storage) missing))
(assert (= (trans-attr |13| |Tamper Protection|) missing))
(assert (= (trans-attr |13| |Token Signing|) missing))
(assert (= (trans-attr |13| |Token Validation|) missing))
(assert (= (trans-attr |13| Troughput) missing))
(assert (= (trans-attr |13| Unit) missing))
(assert (= (trans-attr |13| |Update capabilities|) missing))
(assert (= (trans-attr |13| Updates) missing))
(assert (= (trans-attr |13| |URL Blacklisting|) missing))
(assert (= (trans-attr |13| |User File Upload|) missing))
(assert (= (trans-attr |13| |User Interfaces|) missing))
(assert (= (trans-attr |13| |User Management|) missing))
(assert (= (trans-attr |13| |Wired interface|) missing))
(assert (= (trans-attr |13| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |13| |Wireless Interface|) missing))
(assert (= (transition-type |14|) |Wireless Connector|))
(assert (and (= (source |14|) |3|) (= (target |14|) |12|)))
(assert (or (= (trans-attr |14| Authentication) undefined)
    (= (trans-attr |14| Authentication) strong)
    (= (trans-attr |14| Authentication) Yes)
    (= (trans-attr |14| Authentication) No)
    (= (trans-attr |14| Authentication) undefined)
    (= (trans-attr |14| Authentication) strong)
    (= (trans-attr |14| Authentication) Yes)
    (= (trans-attr |14| Authentication) No)
    (= (trans-attr |14| Authentication) undefined)
    (= (trans-attr |14| Authentication) strong)
    (= (trans-attr |14| Authentication) Yes)
    (= (trans-attr |14| Authentication) No)))
(assert (or (= (trans-attr |14| |Credential Asset|) undefined)
    (= (trans-attr |14| |Credential Asset|) Yes)
    (= (trans-attr |14| |Credential Asset|) No)
    (= (trans-attr |14| |Credential Asset|) encrypted)
    (= (trans-attr |14| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |14| |Credential Asset|) undefined)
    (= (trans-attr |14| |Credential Asset|) Yes)
    (= (trans-attr |14| |Credential Asset|) No)
    (= (trans-attr |14| |Credential Asset|) encrypted)
    (= (trans-attr |14| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |14| |Credential Asset|) undefined)
    (= (trans-attr |14| |Credential Asset|) Yes)
    (= (trans-attr |14| |Credential Asset|) No)
    (= (trans-attr |14| |Credential Asset|) encrypted)
    (= (trans-attr |14| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |14| Encrypted) undefined)
    (= (trans-attr |14| Encrypted) Yes)
    (= (trans-attr |14| Encrypted) No)
    (= (trans-attr |14| Encrypted) strong)
    (= (trans-attr |14| Encrypted) undefined)
    (= (trans-attr |14| Encrypted) Yes)
    (= (trans-attr |14| Encrypted) No)
    (= (trans-attr |14| Encrypted) strong)
    (= (trans-attr |14| Encrypted) undefined)
    (= (trans-attr |14| Encrypted) Yes)
    (= (trans-attr |14| Encrypted) No)
    (= (trans-attr |14| Encrypted) strong)))
(assert (or (= (trans-attr |14| |Encryption Method|) undefined)
    (= (trans-attr |14| |Encryption Method|) strong)
    (= (trans-attr |14| |Encryption Method|) weak)
    (= (trans-attr |14| |Encryption Method|) undefined)
    (= (trans-attr |14| |Encryption Method|) strong)
    (= (trans-attr |14| |Encryption Method|) weak)
    (= (trans-attr |14| |Encryption Method|) undefined)
    (= (trans-attr |14| |Encryption Method|) strong)
    (= (trans-attr |14| |Encryption Method|) weak)))
(assert (= (trans-attr |14| |Access Control|) missing))
(assert (= (trans-attr |14| |Activity Logging|) missing))
(assert (= (trans-attr |14| Administration) missing))
(assert (= (trans-attr |14| |Allows User Input|) missing))
(assert (= (trans-attr |14| |Anomaly Detection|) missing))
(assert (= (trans-attr |14| |API Type|) missing))
(assert (= (trans-attr |14| |Approved License|) missing))
(assert (= (trans-attr |14| Auditing) missing))
(assert (= (trans-attr |14| Authorization) missing))
(assert (= (trans-attr |14| Availability) missing))
(assert (= (trans-attr |14| Bandwidth) missing))
(assert (= (trans-attr |14| |Certificate Checks|) missing))
(assert (= (trans-attr |14| |Coding guideline|) missing))
(assert (= (trans-attr |14| |Communication Latency|) missing))
(assert (= (trans-attr |14| |Communication Reliability|) missing))
(assert (= (trans-attr |14| Confidentiality) missing))
(assert (= (trans-attr |14| Content) missing))
(assert (= (trans-attr |14| |Counterfeit Detection|) missing))
(assert (= (trans-attr |14| Criticality) missing))
(assert (= (trans-attr |14| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |14| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |14| |Data Backup|) missing))
(assert (= (trans-attr |14| |Data safety integrity|) missing))
(assert (= (trans-attr |14| |Data security integrity|) missing))
(assert (= (trans-attr |14| |Data Store|) missing))
(assert (= (trans-attr |14| |DDoS Mitigation|) missing))
(assert (= (trans-attr |14| |Device Fingerprint|) missing))
(assert (= (trans-attr |14| |Digital Signature|) missing))
(assert (= (trans-attr |14| Encryption) missing))
(assert (= (trans-attr |14| |Encryption Time|) missing))
(assert (= (trans-attr |14| |Error Rate|) missing))
(assert (= (trans-attr |14| Feedback) missing))
(assert (= (trans-attr |14| |Financial Asset|) missing))
(assert (= (trans-attr |14| Firmware) missing))
(assert (= (trans-attr |14| |Input Sanitization|) missing))
(assert (= (trans-attr |14| |Input Validation|) missing))
(assert (= (trans-attr |14| Integrity) missing))
(assert (= (trans-attr |14| |Key Length|) missing))
(assert (= (trans-attr |14| |Key Revocation|) missing))
(assert (= (trans-attr |14| Language) missing))
(assert (= (trans-attr |14| License) missing))
(assert (= (trans-attr |14| Location) missing))
(assert (= (trans-attr |14| |Malware Protection|) missing))
(assert (= (trans-attr |14| Managed) missing))
(assert (= (trans-attr |14| |Maximum Value|) missing))
(assert (= (trans-attr |14| |Memory Type|) missing))
(assert (= (trans-attr |14| |Minimum Value|) missing))
(assert (= (trans-attr |14| |Network Technology|) missing))
(assert (= (trans-attr |14| |Operating system|) missing))
(assert (= (trans-attr |14| |Operational Criticality|) missing))
(assert (= (trans-attr |14| Permissions) missing))
(assert (= (trans-attr |14| |Physical Location|) missing))
(assert (= (trans-attr |14| |Power consumption|) missing))
(assert (= (trans-attr |14| |Privacy Asset|) missing))
(assert (= (trans-attr |14| |Processing Time|) missing))
(assert (= (trans-attr |14| |Protected Execution Environment|) missing))
(assert (= (trans-attr |14| |Protocol version|) missing))
(assert (= (trans-attr |14| Protocols) missing))
(assert (= (trans-attr |14| |PtwoP Capability|) missing))
(assert (= (trans-attr |14| Range) missing))
(assert (= (trans-attr |14| Redundancy) missing))
(assert (= (trans-attr |14| |Reset capabilities|) missing))
(assert (= (trans-attr |14| Roles) missing))
(assert (= (trans-attr |14| |Secure Boot|) missing))
(assert (= (trans-attr |14| |Secure Session Handling|) missing))
(assert (= (trans-attr |14| |Secure Storage|) missing))
(assert (= (trans-attr |14| |Secure Update|) missing))
(assert (= (trans-attr |14| |Sensor measurement type|) missing))
(assert (= (trans-attr |14| |Shared resources|) missing))
(assert (= (trans-attr |14| Software) missing))
(assert (= (trans-attr |14| |Software APIs|) missing))
(assert (= (trans-attr |14| |Standard Password|) missing))
(assert (= (trans-attr |14| Storage) missing))
(assert (= (trans-attr |14| |Tamper Protection|) missing))
(assert (= (trans-attr |14| |Token Signing|) missing))
(assert (= (trans-attr |14| |Token Validation|) missing))
(assert (= (trans-attr |14| Troughput) missing))
(assert (= (trans-attr |14| Unit) missing))
(assert (= (trans-attr |14| |Update capabilities|) missing))
(assert (= (trans-attr |14| Updates) missing))
(assert (= (trans-attr |14| |URL Blacklisting|) missing))
(assert (= (trans-attr |14| |User File Upload|) missing))
(assert (= (trans-attr |14| |User Interfaces|) missing))
(assert (= (trans-attr |14| |User Management|) missing))
(assert (= (trans-attr |14| |Wired interface|) missing))
(assert (= (trans-attr |14| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |14| |Wireless Interface|) missing))
(assert (= (transition-type |33|) |Wire Connector|))
(assert (and (= (source |33|) |6|) (= (target |33|) |46|)))
(assert (or (= (trans-attr |33| Authentication) undefined)
    (= (trans-attr |33| Authentication) strong)
    (= (trans-attr |33| Authentication) Yes)
    (= (trans-attr |33| Authentication) No)
    (= (trans-attr |33| Authentication) undefined)
    (= (trans-attr |33| Authentication) strong)
    (= (trans-attr |33| Authentication) Yes)
    (= (trans-attr |33| Authentication) No)
    (= (trans-attr |33| Authentication) undefined)
    (= (trans-attr |33| Authentication) strong)
    (= (trans-attr |33| Authentication) Yes)
    (= (trans-attr |33| Authentication) No)))
(assert (or (= (trans-attr |33| |Credential Asset|) undefined)
    (= (trans-attr |33| |Credential Asset|) Yes)
    (= (trans-attr |33| |Credential Asset|) No)
    (= (trans-attr |33| |Credential Asset|) encrypted)
    (= (trans-attr |33| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |33| |Credential Asset|) undefined)
    (= (trans-attr |33| |Credential Asset|) Yes)
    (= (trans-attr |33| |Credential Asset|) No)
    (= (trans-attr |33| |Credential Asset|) encrypted)
    (= (trans-attr |33| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |33| |Credential Asset|) undefined)
    (= (trans-attr |33| |Credential Asset|) Yes)
    (= (trans-attr |33| |Credential Asset|) No)
    (= (trans-attr |33| |Credential Asset|) encrypted)
    (= (trans-attr |33| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |33| Encrypted) undefined)
    (= (trans-attr |33| Encrypted) Yes)
    (= (trans-attr |33| Encrypted) No)
    (= (trans-attr |33| Encrypted) strong)
    (= (trans-attr |33| Encrypted) undefined)
    (= (trans-attr |33| Encrypted) Yes)
    (= (trans-attr |33| Encrypted) No)
    (= (trans-attr |33| Encrypted) strong)
    (= (trans-attr |33| Encrypted) undefined)
    (= (trans-attr |33| Encrypted) Yes)
    (= (trans-attr |33| Encrypted) No)
    (= (trans-attr |33| Encrypted) strong)))
(assert (or (= (trans-attr |33| |Encryption Method|) undefined)
    (= (trans-attr |33| |Encryption Method|) strong)
    (= (trans-attr |33| |Encryption Method|) weak)
    (= (trans-attr |33| |Encryption Method|) undefined)
    (= (trans-attr |33| |Encryption Method|) strong)
    (= (trans-attr |33| |Encryption Method|) weak)
    (= (trans-attr |33| |Encryption Method|) undefined)
    (= (trans-attr |33| |Encryption Method|) strong)
    (= (trans-attr |33| |Encryption Method|) weak)))
(assert (= (trans-attr |33| |Access Control|) missing))
(assert (= (trans-attr |33| |Activity Logging|) missing))
(assert (= (trans-attr |33| Administration) missing))
(assert (= (trans-attr |33| |Allows User Input|) missing))
(assert (= (trans-attr |33| |Anomaly Detection|) missing))
(assert (= (trans-attr |33| |API Type|) missing))
(assert (= (trans-attr |33| |Approved License|) missing))
(assert (= (trans-attr |33| Auditing) missing))
(assert (= (trans-attr |33| Authorization) missing))
(assert (= (trans-attr |33| Availability) missing))
(assert (= (trans-attr |33| Bandwidth) missing))
(assert (= (trans-attr |33| |Certificate Checks|) missing))
(assert (= (trans-attr |33| |Coding guideline|) missing))
(assert (= (trans-attr |33| |Communication Latency|) missing))
(assert (= (trans-attr |33| |Communication Reliability|) missing))
(assert (= (trans-attr |33| Confidentiality) missing))
(assert (= (trans-attr |33| Content) missing))
(assert (= (trans-attr |33| |Counterfeit Detection|) missing))
(assert (= (trans-attr |33| Criticality) missing))
(assert (= (trans-attr |33| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |33| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |33| |Data Backup|) missing))
(assert (= (trans-attr |33| |Data safety integrity|) missing))
(assert (= (trans-attr |33| |Data security integrity|) missing))
(assert (= (trans-attr |33| |Data Store|) missing))
(assert (= (trans-attr |33| |DDoS Mitigation|) missing))
(assert (= (trans-attr |33| |Device Fingerprint|) missing))
(assert (= (trans-attr |33| |Digital Signature|) missing))
(assert (= (trans-attr |33| Encryption) missing))
(assert (= (trans-attr |33| |Encryption Time|) missing))
(assert (= (trans-attr |33| |Error Rate|) missing))
(assert (= (trans-attr |33| Feedback) missing))
(assert (= (trans-attr |33| |Financial Asset|) missing))
(assert (= (trans-attr |33| Firmware) missing))
(assert (= (trans-attr |33| |Input Sanitization|) missing))
(assert (= (trans-attr |33| |Input Validation|) missing))
(assert (= (trans-attr |33| Integrity) missing))
(assert (= (trans-attr |33| |Key Length|) missing))
(assert (= (trans-attr |33| |Key Revocation|) missing))
(assert (= (trans-attr |33| Language) missing))
(assert (= (trans-attr |33| License) missing))
(assert (= (trans-attr |33| Location) missing))
(assert (= (trans-attr |33| |Malware Protection|) missing))
(assert (= (trans-attr |33| Managed) missing))
(assert (= (trans-attr |33| |Maximum Value|) missing))
(assert (= (trans-attr |33| |Memory Type|) missing))
(assert (= (trans-attr |33| |Minimum Value|) missing))
(assert (= (trans-attr |33| |Network Technology|) missing))
(assert (= (trans-attr |33| |Operating system|) missing))
(assert (= (trans-attr |33| |Operational Criticality|) missing))
(assert (= (trans-attr |33| Permissions) missing))
(assert (= (trans-attr |33| |Physical Location|) missing))
(assert (= (trans-attr |33| |Power consumption|) missing))
(assert (= (trans-attr |33| |Privacy Asset|) missing))
(assert (= (trans-attr |33| |Processing Time|) missing))
(assert (= (trans-attr |33| |Protected Execution Environment|) missing))
(assert (= (trans-attr |33| |Protocol version|) missing))
(assert (= (trans-attr |33| Protocols) missing))
(assert (= (trans-attr |33| |PtwoP Capability|) missing))
(assert (= (trans-attr |33| Range) missing))
(assert (= (trans-attr |33| Redundancy) missing))
(assert (= (trans-attr |33| |Reset capabilities|) missing))
(assert (= (trans-attr |33| Roles) missing))
(assert (= (trans-attr |33| |Secure Boot|) missing))
(assert (= (trans-attr |33| |Secure Session Handling|) missing))
(assert (= (trans-attr |33| |Secure Storage|) missing))
(assert (= (trans-attr |33| |Secure Update|) missing))
(assert (= (trans-attr |33| |Sensor measurement type|) missing))
(assert (= (trans-attr |33| |Shared resources|) missing))
(assert (= (trans-attr |33| Software) missing))
(assert (= (trans-attr |33| |Software APIs|) missing))
(assert (= (trans-attr |33| |Standard Password|) missing))
(assert (= (trans-attr |33| Storage) missing))
(assert (= (trans-attr |33| |Tamper Protection|) missing))
(assert (= (trans-attr |33| |Token Signing|) missing))
(assert (= (trans-attr |33| |Token Validation|) missing))
(assert (= (trans-attr |33| Troughput) missing))
(assert (= (trans-attr |33| Unit) missing))
(assert (= (trans-attr |33| |Update capabilities|) missing))
(assert (= (trans-attr |33| Updates) missing))
(assert (= (trans-attr |33| |URL Blacklisting|) missing))
(assert (= (trans-attr |33| |User File Upload|) missing))
(assert (= (trans-attr |33| |User Interfaces|) missing))
(assert (= (trans-attr |33| |User Management|) missing))
(assert (= (trans-attr |33| |Wired interface|) missing))
(assert (= (trans-attr |33| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |33| |Wireless Interface|) missing))
(assert (= (transition-type |34|) |Wire Connector|))
(assert (and (= (source |34|) |46|) (= (target |34|) |6|)))
(assert (or (= (trans-attr |34| Authentication) undefined)
    (= (trans-attr |34| Authentication) strong)
    (= (trans-attr |34| Authentication) Yes)
    (= (trans-attr |34| Authentication) No)
    (= (trans-attr |34| Authentication) undefined)
    (= (trans-attr |34| Authentication) strong)
    (= (trans-attr |34| Authentication) Yes)
    (= (trans-attr |34| Authentication) No)
    (= (trans-attr |34| Authentication) undefined)
    (= (trans-attr |34| Authentication) strong)
    (= (trans-attr |34| Authentication) Yes)
    (= (trans-attr |34| Authentication) No)))
(assert (or (= (trans-attr |34| |Credential Asset|) undefined)
    (= (trans-attr |34| |Credential Asset|) Yes)
    (= (trans-attr |34| |Credential Asset|) No)
    (= (trans-attr |34| |Credential Asset|) encrypted)
    (= (trans-attr |34| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |34| |Credential Asset|) undefined)
    (= (trans-attr |34| |Credential Asset|) Yes)
    (= (trans-attr |34| |Credential Asset|) No)
    (= (trans-attr |34| |Credential Asset|) encrypted)
    (= (trans-attr |34| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |34| |Credential Asset|) undefined)
    (= (trans-attr |34| |Credential Asset|) Yes)
    (= (trans-attr |34| |Credential Asset|) No)
    (= (trans-attr |34| |Credential Asset|) encrypted)
    (= (trans-attr |34| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |34| Encrypted) undefined)
    (= (trans-attr |34| Encrypted) Yes)
    (= (trans-attr |34| Encrypted) No)
    (= (trans-attr |34| Encrypted) strong)
    (= (trans-attr |34| Encrypted) undefined)
    (= (trans-attr |34| Encrypted) Yes)
    (= (trans-attr |34| Encrypted) No)
    (= (trans-attr |34| Encrypted) strong)
    (= (trans-attr |34| Encrypted) undefined)
    (= (trans-attr |34| Encrypted) Yes)
    (= (trans-attr |34| Encrypted) No)
    (= (trans-attr |34| Encrypted) strong)))
(assert (or (= (trans-attr |34| |Encryption Method|) undefined)
    (= (trans-attr |34| |Encryption Method|) strong)
    (= (trans-attr |34| |Encryption Method|) weak)
    (= (trans-attr |34| |Encryption Method|) undefined)
    (= (trans-attr |34| |Encryption Method|) strong)
    (= (trans-attr |34| |Encryption Method|) weak)
    (= (trans-attr |34| |Encryption Method|) undefined)
    (= (trans-attr |34| |Encryption Method|) strong)
    (= (trans-attr |34| |Encryption Method|) weak)))
(assert (= (trans-attr |34| |Access Control|) missing))
(assert (= (trans-attr |34| |Activity Logging|) missing))
(assert (= (trans-attr |34| Administration) missing))
(assert (= (trans-attr |34| |Allows User Input|) missing))
(assert (= (trans-attr |34| |Anomaly Detection|) missing))
(assert (= (trans-attr |34| |API Type|) missing))
(assert (= (trans-attr |34| |Approved License|) missing))
(assert (= (trans-attr |34| Auditing) missing))
(assert (= (trans-attr |34| Authorization) missing))
(assert (= (trans-attr |34| Availability) missing))
(assert (= (trans-attr |34| Bandwidth) missing))
(assert (= (trans-attr |34| |Certificate Checks|) missing))
(assert (= (trans-attr |34| |Coding guideline|) missing))
(assert (= (trans-attr |34| |Communication Latency|) missing))
(assert (= (trans-attr |34| |Communication Reliability|) missing))
(assert (= (trans-attr |34| Confidentiality) missing))
(assert (= (trans-attr |34| Content) missing))
(assert (= (trans-attr |34| |Counterfeit Detection|) missing))
(assert (= (trans-attr |34| Criticality) missing))
(assert (= (trans-attr |34| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |34| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |34| |Data Backup|) missing))
(assert (= (trans-attr |34| |Data safety integrity|) missing))
(assert (= (trans-attr |34| |Data security integrity|) missing))
(assert (= (trans-attr |34| |Data Store|) missing))
(assert (= (trans-attr |34| |DDoS Mitigation|) missing))
(assert (= (trans-attr |34| |Device Fingerprint|) missing))
(assert (= (trans-attr |34| |Digital Signature|) missing))
(assert (= (trans-attr |34| Encryption) missing))
(assert (= (trans-attr |34| |Encryption Time|) missing))
(assert (= (trans-attr |34| |Error Rate|) missing))
(assert (= (trans-attr |34| Feedback) missing))
(assert (= (trans-attr |34| |Financial Asset|) missing))
(assert (= (trans-attr |34| Firmware) missing))
(assert (= (trans-attr |34| |Input Sanitization|) missing))
(assert (= (trans-attr |34| |Input Validation|) missing))
(assert (= (trans-attr |34| Integrity) missing))
(assert (= (trans-attr |34| |Key Length|) missing))
(assert (= (trans-attr |34| |Key Revocation|) missing))
(assert (= (trans-attr |34| Language) missing))
(assert (= (trans-attr |34| License) missing))
(assert (= (trans-attr |34| Location) missing))
(assert (= (trans-attr |34| |Malware Protection|) missing))
(assert (= (trans-attr |34| Managed) missing))
(assert (= (trans-attr |34| |Maximum Value|) missing))
(assert (= (trans-attr |34| |Memory Type|) missing))
(assert (= (trans-attr |34| |Minimum Value|) missing))
(assert (= (trans-attr |34| |Network Technology|) missing))
(assert (= (trans-attr |34| |Operating system|) missing))
(assert (= (trans-attr |34| |Operational Criticality|) missing))
(assert (= (trans-attr |34| Permissions) missing))
(assert (= (trans-attr |34| |Physical Location|) missing))
(assert (= (trans-attr |34| |Power consumption|) missing))
(assert (= (trans-attr |34| |Privacy Asset|) missing))
(assert (= (trans-attr |34| |Processing Time|) missing))
(assert (= (trans-attr |34| |Protected Execution Environment|) missing))
(assert (= (trans-attr |34| |Protocol version|) missing))
(assert (= (trans-attr |34| Protocols) missing))
(assert (= (trans-attr |34| |PtwoP Capability|) missing))
(assert (= (trans-attr |34| Range) missing))
(assert (= (trans-attr |34| Redundancy) missing))
(assert (= (trans-attr |34| |Reset capabilities|) missing))
(assert (= (trans-attr |34| Roles) missing))
(assert (= (trans-attr |34| |Secure Boot|) missing))
(assert (= (trans-attr |34| |Secure Session Handling|) missing))
(assert (= (trans-attr |34| |Secure Storage|) missing))
(assert (= (trans-attr |34| |Secure Update|) missing))
(assert (= (trans-attr |34| |Sensor measurement type|) missing))
(assert (= (trans-attr |34| |Shared resources|) missing))
(assert (= (trans-attr |34| Software) missing))
(assert (= (trans-attr |34| |Software APIs|) missing))
(assert (= (trans-attr |34| |Standard Password|) missing))
(assert (= (trans-attr |34| Storage) missing))
(assert (= (trans-attr |34| |Tamper Protection|) missing))
(assert (= (trans-attr |34| |Token Signing|) missing))
(assert (= (trans-attr |34| |Token Validation|) missing))
(assert (= (trans-attr |34| Troughput) missing))
(assert (= (trans-attr |34| Unit) missing))
(assert (= (trans-attr |34| |Update capabilities|) missing))
(assert (= (trans-attr |34| Updates) missing))
(assert (= (trans-attr |34| |URL Blacklisting|) missing))
(assert (= (trans-attr |34| |User File Upload|) missing))
(assert (= (trans-attr |34| |User Interfaces|) missing))
(assert (= (trans-attr |34| |User Management|) missing))
(assert (= (trans-attr |34| |Wired interface|) missing))
(assert (= (trans-attr |34| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |34| |Wireless Interface|) missing))
(assert (= (transition-type |36|) |Wire Connector|))
(assert (and (= (source |36|) |46|) (= (target |36|) |12|)))
(assert (or (= (trans-attr |36| Authentication) undefined)
    (= (trans-attr |36| Authentication) strong)
    (= (trans-attr |36| Authentication) Yes)
    (= (trans-attr |36| Authentication) No)
    (= (trans-attr |36| Authentication) undefined)
    (= (trans-attr |36| Authentication) strong)
    (= (trans-attr |36| Authentication) Yes)
    (= (trans-attr |36| Authentication) No)
    (= (trans-attr |36| Authentication) undefined)
    (= (trans-attr |36| Authentication) strong)
    (= (trans-attr |36| Authentication) Yes)
    (= (trans-attr |36| Authentication) No)))
(assert (or (= (trans-attr |36| |Credential Asset|) undefined)
    (= (trans-attr |36| |Credential Asset|) Yes)
    (= (trans-attr |36| |Credential Asset|) No)
    (= (trans-attr |36| |Credential Asset|) encrypted)
    (= (trans-attr |36| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |36| |Credential Asset|) undefined)
    (= (trans-attr |36| |Credential Asset|) Yes)
    (= (trans-attr |36| |Credential Asset|) No)
    (= (trans-attr |36| |Credential Asset|) encrypted)
    (= (trans-attr |36| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |36| |Credential Asset|) undefined)
    (= (trans-attr |36| |Credential Asset|) Yes)
    (= (trans-attr |36| |Credential Asset|) No)
    (= (trans-attr |36| |Credential Asset|) encrypted)
    (= (trans-attr |36| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |36| Encrypted) undefined)
    (= (trans-attr |36| Encrypted) Yes)
    (= (trans-attr |36| Encrypted) No)
    (= (trans-attr |36| Encrypted) strong)
    (= (trans-attr |36| Encrypted) undefined)
    (= (trans-attr |36| Encrypted) Yes)
    (= (trans-attr |36| Encrypted) No)
    (= (trans-attr |36| Encrypted) strong)
    (= (trans-attr |36| Encrypted) undefined)
    (= (trans-attr |36| Encrypted) Yes)
    (= (trans-attr |36| Encrypted) No)
    (= (trans-attr |36| Encrypted) strong)))
(assert (or (= (trans-attr |36| |Encryption Method|) undefined)
    (= (trans-attr |36| |Encryption Method|) strong)
    (= (trans-attr |36| |Encryption Method|) weak)
    (= (trans-attr |36| |Encryption Method|) undefined)
    (= (trans-attr |36| |Encryption Method|) strong)
    (= (trans-attr |36| |Encryption Method|) weak)
    (= (trans-attr |36| |Encryption Method|) undefined)
    (= (trans-attr |36| |Encryption Method|) strong)
    (= (trans-attr |36| |Encryption Method|) weak)))
(assert (= (trans-attr |36| |Access Control|) missing))
(assert (= (trans-attr |36| |Activity Logging|) missing))
(assert (= (trans-attr |36| Administration) missing))
(assert (= (trans-attr |36| |Allows User Input|) missing))
(assert (= (trans-attr |36| |Anomaly Detection|) missing))
(assert (= (trans-attr |36| |API Type|) missing))
(assert (= (trans-attr |36| |Approved License|) missing))
(assert (= (trans-attr |36| Auditing) missing))
(assert (= (trans-attr |36| Authorization) missing))
(assert (= (trans-attr |36| Availability) missing))
(assert (= (trans-attr |36| Bandwidth) missing))
(assert (= (trans-attr |36| |Certificate Checks|) missing))
(assert (= (trans-attr |36| |Coding guideline|) missing))
(assert (= (trans-attr |36| |Communication Latency|) missing))
(assert (= (trans-attr |36| |Communication Reliability|) missing))
(assert (= (trans-attr |36| Confidentiality) missing))
(assert (= (trans-attr |36| Content) missing))
(assert (= (trans-attr |36| |Counterfeit Detection|) missing))
(assert (= (trans-attr |36| Criticality) missing))
(assert (= (trans-attr |36| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |36| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |36| |Data Backup|) missing))
(assert (= (trans-attr |36| |Data safety integrity|) missing))
(assert (= (trans-attr |36| |Data security integrity|) missing))
(assert (= (trans-attr |36| |Data Store|) missing))
(assert (= (trans-attr |36| |DDoS Mitigation|) missing))
(assert (= (trans-attr |36| |Device Fingerprint|) missing))
(assert (= (trans-attr |36| |Digital Signature|) missing))
(assert (= (trans-attr |36| Encryption) missing))
(assert (= (trans-attr |36| |Encryption Time|) missing))
(assert (= (trans-attr |36| |Error Rate|) missing))
(assert (= (trans-attr |36| Feedback) missing))
(assert (= (trans-attr |36| |Financial Asset|) missing))
(assert (= (trans-attr |36| Firmware) missing))
(assert (= (trans-attr |36| |Input Sanitization|) missing))
(assert (= (trans-attr |36| |Input Validation|) missing))
(assert (= (trans-attr |36| Integrity) missing))
(assert (= (trans-attr |36| |Key Length|) missing))
(assert (= (trans-attr |36| |Key Revocation|) missing))
(assert (= (trans-attr |36| Language) missing))
(assert (= (trans-attr |36| License) missing))
(assert (= (trans-attr |36| Location) missing))
(assert (= (trans-attr |36| |Malware Protection|) missing))
(assert (= (trans-attr |36| Managed) missing))
(assert (= (trans-attr |36| |Maximum Value|) missing))
(assert (= (trans-attr |36| |Memory Type|) missing))
(assert (= (trans-attr |36| |Minimum Value|) missing))
(assert (= (trans-attr |36| |Network Technology|) missing))
(assert (= (trans-attr |36| |Operating system|) missing))
(assert (= (trans-attr |36| |Operational Criticality|) missing))
(assert (= (trans-attr |36| Permissions) missing))
(assert (= (trans-attr |36| |Physical Location|) missing))
(assert (= (trans-attr |36| |Power consumption|) missing))
(assert (= (trans-attr |36| |Privacy Asset|) missing))
(assert (= (trans-attr |36| |Processing Time|) missing))
(assert (= (trans-attr |36| |Protected Execution Environment|) missing))
(assert (= (trans-attr |36| |Protocol version|) missing))
(assert (= (trans-attr |36| Protocols) missing))
(assert (= (trans-attr |36| |PtwoP Capability|) missing))
(assert (= (trans-attr |36| Range) missing))
(assert (= (trans-attr |36| Redundancy) missing))
(assert (= (trans-attr |36| |Reset capabilities|) missing))
(assert (= (trans-attr |36| Roles) missing))
(assert (= (trans-attr |36| |Secure Boot|) missing))
(assert (= (trans-attr |36| |Secure Session Handling|) missing))
(assert (= (trans-attr |36| |Secure Storage|) missing))
(assert (= (trans-attr |36| |Secure Update|) missing))
(assert (= (trans-attr |36| |Sensor measurement type|) missing))
(assert (= (trans-attr |36| |Shared resources|) missing))
(assert (= (trans-attr |36| Software) missing))
(assert (= (trans-attr |36| |Software APIs|) missing))
(assert (= (trans-attr |36| |Standard Password|) missing))
(assert (= (trans-attr |36| Storage) missing))
(assert (= (trans-attr |36| |Tamper Protection|) missing))
(assert (= (trans-attr |36| |Token Signing|) missing))
(assert (= (trans-attr |36| |Token Validation|) missing))
(assert (= (trans-attr |36| Troughput) missing))
(assert (= (trans-attr |36| Unit) missing))
(assert (= (trans-attr |36| |Update capabilities|) missing))
(assert (= (trans-attr |36| Updates) missing))
(assert (= (trans-attr |36| |URL Blacklisting|) missing))
(assert (= (trans-attr |36| |User File Upload|) missing))
(assert (= (trans-attr |36| |User Interfaces|) missing))
(assert (= (trans-attr |36| |User Management|) missing))
(assert (= (trans-attr |36| |Wired interface|) missing))
(assert (= (trans-attr |36| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |36| |Wireless Interface|) missing))
(assert (= (transition-type |39|) |Wire Connector|))
(assert (and (= (source |39|) |12|) (= (target |39|) |46|)))
(assert (or (= (trans-attr |39| Authentication) undefined)
    (= (trans-attr |39| Authentication) strong)
    (= (trans-attr |39| Authentication) Yes)
    (= (trans-attr |39| Authentication) No)
    (= (trans-attr |39| Authentication) undefined)
    (= (trans-attr |39| Authentication) strong)
    (= (trans-attr |39| Authentication) Yes)
    (= (trans-attr |39| Authentication) No)
    (= (trans-attr |39| Authentication) undefined)
    (= (trans-attr |39| Authentication) strong)
    (= (trans-attr |39| Authentication) Yes)
    (= (trans-attr |39| Authentication) No)))
(assert (or (= (trans-attr |39| |Credential Asset|) undefined)
    (= (trans-attr |39| |Credential Asset|) Yes)
    (= (trans-attr |39| |Credential Asset|) No)
    (= (trans-attr |39| |Credential Asset|) encrypted)
    (= (trans-attr |39| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |39| |Credential Asset|) undefined)
    (= (trans-attr |39| |Credential Asset|) Yes)
    (= (trans-attr |39| |Credential Asset|) No)
    (= (trans-attr |39| |Credential Asset|) encrypted)
    (= (trans-attr |39| |Credential Asset|) |salted and hashed|)
    (= (trans-attr |39| |Credential Asset|) undefined)
    (= (trans-attr |39| |Credential Asset|) Yes)
    (= (trans-attr |39| |Credential Asset|) No)
    (= (trans-attr |39| |Credential Asset|) encrypted)
    (= (trans-attr |39| |Credential Asset|) |salted and hashed|)))
(assert (or (= (trans-attr |39| Encrypted) undefined)
    (= (trans-attr |39| Encrypted) Yes)
    (= (trans-attr |39| Encrypted) No)
    (= (trans-attr |39| Encrypted) strong)
    (= (trans-attr |39| Encrypted) undefined)
    (= (trans-attr |39| Encrypted) Yes)
    (= (trans-attr |39| Encrypted) No)
    (= (trans-attr |39| Encrypted) strong)
    (= (trans-attr |39| Encrypted) undefined)
    (= (trans-attr |39| Encrypted) Yes)
    (= (trans-attr |39| Encrypted) No)
    (= (trans-attr |39| Encrypted) strong)))
(assert (or (= (trans-attr |39| |Encryption Method|) undefined)
    (= (trans-attr |39| |Encryption Method|) strong)
    (= (trans-attr |39| |Encryption Method|) weak)
    (= (trans-attr |39| |Encryption Method|) undefined)
    (= (trans-attr |39| |Encryption Method|) strong)
    (= (trans-attr |39| |Encryption Method|) weak)
    (= (trans-attr |39| |Encryption Method|) undefined)
    (= (trans-attr |39| |Encryption Method|) strong)
    (= (trans-attr |39| |Encryption Method|) weak)))
(assert (= (trans-attr |39| |Access Control|) missing))
(assert (= (trans-attr |39| |Activity Logging|) missing))
(assert (= (trans-attr |39| Administration) missing))
(assert (= (trans-attr |39| |Allows User Input|) missing))
(assert (= (trans-attr |39| |Anomaly Detection|) missing))
(assert (= (trans-attr |39| |API Type|) missing))
(assert (= (trans-attr |39| |Approved License|) missing))
(assert (= (trans-attr |39| Auditing) missing))
(assert (= (trans-attr |39| Authorization) missing))
(assert (= (trans-attr |39| Availability) missing))
(assert (= (trans-attr |39| Bandwidth) missing))
(assert (= (trans-attr |39| |Certificate Checks|) missing))
(assert (= (trans-attr |39| |Coding guideline|) missing))
(assert (= (trans-attr |39| |Communication Latency|) missing))
(assert (= (trans-attr |39| |Communication Reliability|) missing))
(assert (= (trans-attr |39| Confidentiality) missing))
(assert (= (trans-attr |39| Content) missing))
(assert (= (trans-attr |39| |Counterfeit Detection|) missing))
(assert (= (trans-attr |39| Criticality) missing))
(assert (= (trans-attr |39| |Cryptographic Algorithms|) missing))
(assert (= (trans-attr |39| |Cryptographic Hardware|) missing))
(assert (= (trans-attr |39| |Data Backup|) missing))
(assert (= (trans-attr |39| |Data safety integrity|) missing))
(assert (= (trans-attr |39| |Data security integrity|) missing))
(assert (= (trans-attr |39| |Data Store|) missing))
(assert (= (trans-attr |39| |DDoS Mitigation|) missing))
(assert (= (trans-attr |39| |Device Fingerprint|) missing))
(assert (= (trans-attr |39| |Digital Signature|) missing))
(assert (= (trans-attr |39| Encryption) missing))
(assert (= (trans-attr |39| |Encryption Time|) missing))
(assert (= (trans-attr |39| |Error Rate|) missing))
(assert (= (trans-attr |39| Feedback) missing))
(assert (= (trans-attr |39| |Financial Asset|) missing))
(assert (= (trans-attr |39| Firmware) missing))
(assert (= (trans-attr |39| |Input Sanitization|) missing))
(assert (= (trans-attr |39| |Input Validation|) missing))
(assert (= (trans-attr |39| Integrity) missing))
(assert (= (trans-attr |39| |Key Length|) missing))
(assert (= (trans-attr |39| |Key Revocation|) missing))
(assert (= (trans-attr |39| Language) missing))
(assert (= (trans-attr |39| License) missing))
(assert (= (trans-attr |39| Location) missing))
(assert (= (trans-attr |39| |Malware Protection|) missing))
(assert (= (trans-attr |39| Managed) missing))
(assert (= (trans-attr |39| |Maximum Value|) missing))
(assert (= (trans-attr |39| |Memory Type|) missing))
(assert (= (trans-attr |39| |Minimum Value|) missing))
(assert (= (trans-attr |39| |Network Technology|) missing))
(assert (= (trans-attr |39| |Operating system|) missing))
(assert (= (trans-attr |39| |Operational Criticality|) missing))
(assert (= (trans-attr |39| Permissions) missing))
(assert (= (trans-attr |39| |Physical Location|) missing))
(assert (= (trans-attr |39| |Power consumption|) missing))
(assert (= (trans-attr |39| |Privacy Asset|) missing))
(assert (= (trans-attr |39| |Processing Time|) missing))
(assert (= (trans-attr |39| |Protected Execution Environment|) missing))
(assert (= (trans-attr |39| |Protocol version|) missing))
(assert (= (trans-attr |39| Protocols) missing))
(assert (= (trans-attr |39| |PtwoP Capability|) missing))
(assert (= (trans-attr |39| Range) missing))
(assert (= (trans-attr |39| Redundancy) missing))
(assert (= (trans-attr |39| |Reset capabilities|) missing))
(assert (= (trans-attr |39| Roles) missing))
(assert (= (trans-attr |39| |Secure Boot|) missing))
(assert (= (trans-attr |39| |Secure Session Handling|) missing))
(assert (= (trans-attr |39| |Secure Storage|) missing))
(assert (= (trans-attr |39| |Secure Update|) missing))
(assert (= (trans-attr |39| |Sensor measurement type|) missing))
(assert (= (trans-attr |39| |Shared resources|) missing))
(assert (= (trans-attr |39| Software) missing))
(assert (= (trans-attr |39| |Software APIs|) missing))
(assert (= (trans-attr |39| |Standard Password|) missing))
(assert (= (trans-attr |39| Storage) missing))
(assert (= (trans-attr |39| |Tamper Protection|) missing))
(assert (= (trans-attr |39| |Token Signing|) missing))
(assert (= (trans-attr |39| |Token Validation|) missing))
(assert (= (trans-attr |39| Troughput) missing))
(assert (= (trans-attr |39| Unit) missing))
(assert (= (trans-attr |39| |Update capabilities|) missing))
(assert (= (trans-attr |39| Updates) missing))
(assert (= (trans-attr |39| |URL Blacklisting|) missing))
(assert (= (trans-attr |39| |User File Upload|) missing))
(assert (= (trans-attr |39| |User Interfaces|) missing))
(assert (= (trans-attr |39| |User Management|) missing))
(assert (= (trans-attr |39| |Wired interface|) missing))
(assert (= (trans-attr |39| |Wireless Communication Technologie|) missing))
(assert (= (trans-attr |39| |Wireless Interface|) missing))
(assert (let ((a!1 (store (store (store ((as const
                                     (Array asset-trans-relation-sort Bool))
                                  false)
                                (asset-trans-relation-sort |30| |13|)
                                true)
                         (asset-trans-relation-sort |41| |13|)
                         true)
                  (asset-trans-relation-sort |30| |14|)
                  true)))
(let ((a!2 (store (store (store a!1 (asset-trans-relation-sort |41| |14|) true)
                         (asset-trans-relation-sort |30| |36|)
                         true)
                  (asset-trans-relation-sort |41| |36|)
                  true)))
  (= (store (store a!2 (asset-trans-relation-sort |30| |39|) true)
            (asset-trans-relation-sort |41| |39|)
            true)
     asset-trans-relation))))
(assert (= (asset-type |30|) |Confidentiality Asset|))
(assert (= (asset-attr |30| |Access Control|) missing))
(assert (= (asset-attr |30| |Activity Logging|) missing))
(assert (= (asset-attr |30| Administration) missing))
(assert (= (asset-attr |30| |Allows User Input|) missing))
(assert (= (asset-attr |30| |Anomaly Detection|) missing))
(assert (= (asset-attr |30| |API Type|) missing))
(assert (= (asset-attr |30| |Approved License|) missing))
(assert (= (asset-attr |30| Auditing) missing))
(assert (= (asset-attr |30| Authentication) missing))
(assert (= (asset-attr |30| Authorization) missing))
(assert (= (asset-attr |30| Availability) missing))
(assert (= (asset-attr |30| Bandwidth) missing))
(assert (= (asset-attr |30| |Certificate Checks|) missing))
(assert (= (asset-attr |30| |Coding guideline|) missing))
(assert (= (asset-attr |30| |Communication Latency|) missing))
(assert (= (asset-attr |30| |Communication Reliability|) missing))
(assert (= (asset-attr |30| Confidentiality) missing))
(assert (= (asset-attr |30| Content) missing))
(assert (= (asset-attr |30| |Counterfeit Detection|) missing))
(assert (= (asset-attr |30| |Credential Asset|) missing))
(assert (= (asset-attr |30| Criticality) missing))
(assert (= (asset-attr |30| |Cryptographic Algorithms|) missing))
(assert (= (asset-attr |30| |Cryptographic Hardware|) missing))
(assert (= (asset-attr |30| |Data Backup|) missing))
(assert (= (asset-attr |30| |Data safety integrity|) missing))
(assert (= (asset-attr |30| |Data security integrity|) missing))
(assert (= (asset-attr |30| |Data Store|) missing))
(assert (= (asset-attr |30| |DDoS Mitigation|) missing))
(assert (= (asset-attr |30| |Device Fingerprint|) missing))
(assert (= (asset-attr |30| |Digital Signature|) missing))
(assert (= (asset-attr |30| Encryption) missing))
(assert (= (asset-attr |30| |Encryption Method|) missing))
(assert (= (asset-attr |30| |Encryption Time|) missing))
(assert (= (asset-attr |30| |Error Rate|) missing))
(assert (= (asset-attr |30| Feedback) missing))
(assert (= (asset-attr |30| |Financial Asset|) missing))
(assert (= (asset-attr |30| Firmware) missing))
(assert (= (asset-attr |30| |Input Sanitization|) missing))
(assert (= (asset-attr |30| |Input Validation|) missing))
(assert (= (asset-attr |30| Integrity) missing))
(assert (= (asset-attr |30| |Key Length|) missing))
(assert (= (asset-attr |30| |Key Revocation|) missing))
(assert (= (asset-attr |30| Language) missing))
(assert (= (asset-attr |30| License) missing))
(assert (= (asset-attr |30| Location) missing))
(assert (= (asset-attr |30| |Malware Protection|) missing))
(assert (= (asset-attr |30| Managed) missing))
(assert (= (asset-attr |30| |Maximum Value|) missing))
(assert (= (asset-attr |30| |Memory Type|) missing))
(assert (= (asset-attr |30| |Minimum Value|) missing))
(assert (= (asset-attr |30| |Network Technology|) missing))
(assert (= (asset-attr |30| |Operating system|) missing))
(assert (= (asset-attr |30| |Operational Criticality|) missing))
(assert (= (asset-attr |30| Permissions) missing))
(assert (= (asset-attr |30| |Physical Location|) missing))
(assert (= (asset-attr |30| |Power consumption|) missing))
(assert (= (asset-attr |30| |Privacy Asset|) missing))
(assert (= (asset-attr |30| |Processing Time|) missing))
(assert (= (asset-attr |30| |Protected Execution Environment|) missing))
(assert (= (asset-attr |30| |Protocol version|) missing))
(assert (= (asset-attr |30| Protocols) missing))
(assert (= (asset-attr |30| |PtwoP Capability|) missing))
(assert (= (asset-attr |30| Range) missing))
(assert (= (asset-attr |30| Redundancy) missing))
(assert (= (asset-attr |30| |Reset capabilities|) missing))
(assert (= (asset-attr |30| Roles) missing))
(assert (= (asset-attr |30| |Secure Boot|) missing))
(assert (= (asset-attr |30| |Secure Session Handling|) missing))
(assert (= (asset-attr |30| |Secure Storage|) missing))
(assert (= (asset-attr |30| |Secure Update|) missing))
(assert (= (asset-attr |30| |Sensor measurement type|) missing))
(assert (= (asset-attr |30| |Shared resources|) missing))
(assert (= (asset-attr |30| Software) missing))
(assert (= (asset-attr |30| |Software APIs|) missing))
(assert (= (asset-attr |30| |Standard Password|) missing))
(assert (= (asset-attr |30| Storage) missing))
(assert (= (asset-attr |30| |Tamper Protection|) missing))
(assert (= (asset-attr |30| |Token Signing|) missing))
(assert (= (asset-attr |30| |Token Validation|) missing))
(assert (= (asset-attr |30| Troughput) missing))
(assert (= (asset-attr |30| Unit) missing))
(assert (= (asset-attr |30| |Update capabilities|) missing))
(assert (= (asset-attr |30| Updates) missing))
(assert (= (asset-attr |30| |URL Blacklisting|) missing))
(assert (= (asset-attr |30| |User File Upload|) missing))
(assert (= (asset-attr |30| |User Interfaces|) missing))
(assert (= (asset-attr |30| |User Management|) missing))
(assert (= (asset-attr |30| |Wired interface|) missing))
(assert (= (asset-attr |30| |Wireless Communication Technologie|) missing))
(assert (= (asset-attr |30| |Wireless Interface|) missing))
(assert (= (asset-type |41|) |Cryptographic Asset|))
(assert (= (asset-attr |41| |Access Control|) missing))
(assert (= (asset-attr |41| |Activity Logging|) missing))
(assert (= (asset-attr |41| Administration) missing))
(assert (= (asset-attr |41| |Allows User Input|) missing))
(assert (= (asset-attr |41| |Anomaly Detection|) missing))
(assert (= (asset-attr |41| |API Type|) missing))
(assert (= (asset-attr |41| |Approved License|) missing))
(assert (= (asset-attr |41| Auditing) missing))
(assert (= (asset-attr |41| Authentication) missing))
(assert (= (asset-attr |41| Authorization) missing))
(assert (= (asset-attr |41| Availability) missing))
(assert (= (asset-attr |41| Bandwidth) missing))
(assert (= (asset-attr |41| |Certificate Checks|) missing))
(assert (= (asset-attr |41| |Coding guideline|) missing))
(assert (= (asset-attr |41| |Communication Latency|) missing))
(assert (= (asset-attr |41| |Communication Reliability|) missing))
(assert (= (asset-attr |41| Confidentiality) missing))
(assert (= (asset-attr |41| Content) missing))
(assert (= (asset-attr |41| |Counterfeit Detection|) missing))
(assert (= (asset-attr |41| |Credential Asset|) missing))
(assert (= (asset-attr |41| Criticality) missing))
(assert (= (asset-attr |41| |Cryptographic Algorithms|) missing))
(assert (= (asset-attr |41| |Cryptographic Hardware|) missing))
(assert (= (asset-attr |41| |Data Backup|) missing))
(assert (= (asset-attr |41| |Data safety integrity|) missing))
(assert (= (asset-attr |41| |Data security integrity|) missing))
(assert (= (asset-attr |41| |Data Store|) missing))
(assert (= (asset-attr |41| |DDoS Mitigation|) missing))
(assert (= (asset-attr |41| |Device Fingerprint|) missing))
(assert (= (asset-attr |41| |Digital Signature|) missing))
(assert (= (asset-attr |41| Encryption) missing))
(assert (= (asset-attr |41| |Encryption Method|) missing))
(assert (= (asset-attr |41| |Encryption Time|) missing))
(assert (= (asset-attr |41| |Error Rate|) missing))
(assert (= (asset-attr |41| Feedback) missing))
(assert (= (asset-attr |41| |Financial Asset|) missing))
(assert (= (asset-attr |41| Firmware) missing))
(assert (= (asset-attr |41| |Input Sanitization|) missing))
(assert (= (asset-attr |41| |Input Validation|) missing))
(assert (= (asset-attr |41| Integrity) missing))
(assert (= (asset-attr |41| |Key Length|) missing))
(assert (= (asset-attr |41| |Key Revocation|) missing))
(assert (= (asset-attr |41| Language) missing))
(assert (= (asset-attr |41| License) missing))
(assert (= (asset-attr |41| Location) missing))
(assert (= (asset-attr |41| |Malware Protection|) missing))
(assert (= (asset-attr |41| Managed) missing))
(assert (= (asset-attr |41| |Maximum Value|) missing))
(assert (= (asset-attr |41| |Memory Type|) missing))
(assert (= (asset-attr |41| |Minimum Value|) missing))
(assert (= (asset-attr |41| |Network Technology|) missing))
(assert (= (asset-attr |41| |Operating system|) missing))
(assert (= (asset-attr |41| |Operational Criticality|) missing))
(assert (= (asset-attr |41| Permissions) missing))
(assert (= (asset-attr |41| |Physical Location|) missing))
(assert (= (asset-attr |41| |Power consumption|) missing))
(assert (= (asset-attr |41| |Privacy Asset|) missing))
(assert (= (asset-attr |41| |Processing Time|) missing))
(assert (= (asset-attr |41| |Protected Execution Environment|) missing))
(assert (= (asset-attr |41| |Protocol version|) missing))
(assert (= (asset-attr |41| Protocols) missing))
(assert (= (asset-attr |41| |PtwoP Capability|) missing))
(assert (= (asset-attr |41| Range) missing))
(assert (= (asset-attr |41| Redundancy) missing))
(assert (= (asset-attr |41| |Reset capabilities|) missing))
(assert (= (asset-attr |41| Roles) missing))
(assert (= (asset-attr |41| |Secure Boot|) missing))
(assert (= (asset-attr |41| |Secure Session Handling|) missing))
(assert (= (asset-attr |41| |Secure Storage|) missing))
(assert (= (asset-attr |41| |Secure Update|) missing))
(assert (= (asset-attr |41| |Sensor measurement type|) missing))
(assert (= (asset-attr |41| |Shared resources|) missing))
(assert (= (asset-attr |41| Software) missing))
(assert (= (asset-attr |41| |Software APIs|) missing))
(assert (= (asset-attr |41| |Standard Password|) missing))
(assert (= (asset-attr |41| Storage) missing))
(assert (= (asset-attr |41| |Tamper Protection|) missing))
(assert (= (asset-attr |41| |Token Signing|) missing))
(assert (= (asset-attr |41| |Token Validation|) missing))
(assert (= (asset-attr |41| Troughput) missing))
(assert (= (asset-attr |41| Unit) missing))
(assert (= (asset-attr |41| |Update capabilities|) missing))
(assert (= (asset-attr |41| Updates) missing))
(assert (= (asset-attr |41| |URL Blacklisting|) missing))
(assert (= (asset-attr |41| |User File Upload|) missing))
(assert (= (asset-attr |41| |User Interfaces|) missing))
(assert (= (asset-attr |41| |User Management|) missing))
(assert (= (asset-attr |41| |Wired interface|) missing))
(assert (= (asset-attr |41| |Wireless Communication Technologie|) missing))
(assert (= (asset-attr |41| |Wireless Interface|) missing))

\end{lstlisting}

==> content/related/adt.tex <==
\subsection{Attack and Attack-Defense Trees}
% Attack Trees
Attack trees model complex attacks through a tree whose root represents the target of the attacker  and whose leaves capture basic attack steps. The remaining nodes, called gates, are either of type AND or type OR and describe which of the sub-goals represented by their children need to be achieved to be able to move closer towards the target. AND-nodes require all the sub-goals to be achieved while for OR-nodes one achieved sub-goal is already enough to proceed. Every path from a leaf to the target node represents a potential attack and this attack can be phrased in terms of Boolean formulas. While attack trees have been used in practice for quite a while, a formal description is relatively new \cite{Mauw2006}. Extensions of standard attack trees allows sequential conjunctions to model situations where timing of events matters \cite{Bryans2019}. 
%Generation of attack trees may be supported by tools such as AttackTree by Isograph [Isograph, 2020] or SecurITree [SecurITree, 2020]. AttackTree offers a graphical representation to support threat analysis and risk assessment (following the corresponding ISO standards). SecurITree similarly offers a graphical interface and lets user assign parameters to nodes to measure resources or resulting impact. 
Attack trees are relatively new to the automotive domain. In the context of vehicle security, one can generate attack trees to automatically generate tests to make cars more secure \cite{Cheah2018}. Attacks on modern vehicles are converted into attack trees in \cite{Karray2018} in order to estimate the overall risk on the system with the aim to build more secure architectures.

% Attack Trees with Attributes
Attack trees support the analysis of attributes of attacks, such as possibility, cost, or resources \cite{Mauw2006}. Such attribute values are assigned to the leaves that represent the basic attack steps. At intermediate nodes, the values of the attributes are synthesized from the children depending on the type of the node. The resulting values enable quantitative reasoning about attacks, particularly, it is possible to investigate which attacks are most costly \cite{Kumar2017} or which attacks can be performed with a certain amount of resources. An overview on the application of formal methods for security models based on attack trees is given in \cite{Widel2019}, focusing on the semantics, generation and analysis of attack trees. Attack-fault trees is a related model that combines description of attack and fault \change{patterns}. A translation of attack-fault trees into parametric weighted timed automata is proposed in~\cite{DBLP:conf/acsd/AndreLRS19}, together with a verification algorithm that allows synthesizing parameters required to perform a successful attack. 

% Attack-Defense Trees
An important missing feature in attack trees is information about the defender’s actions and her potential interaction with the attacker. Attack-defense trees (ADTs) extend attack trees with defense nodes that allow specifying mitigation actions in the model. A formal description of ADTs is given in \cite{Kordy2011} and several semantics have been presented. %Attack-defense trees may also carry attributes.
Recent applications of ADTs include identification of an optimal set of countermeasures to secure a system against several distinct attacks \cite{Fila2020}. Reasonable strategies for both attacker and defender are extracted from an ADT and are input to an optimization framework based on integer linear programming that determines optimal countermeasures.

\change{
Attack and attack-defense trees provide an alternative approach 
to threat modelling and analysis that focuses more on the attacker then on the system to protect. Attack and attack-defence trees have a more dynamic flavour in the sense that they describe sequences of steps to perform a concrete attack in a system. This is in contrast to our approach, 
in which threat rules rather describe structural weaknesses in 
system architectures with respect to security properties.
}
% Representation of Attack Trees Through Timed Automata
%Analysis of attack trees can be supported by timed automata models. Timed automata are finite state machines with clocks that keep track of the time [Alur, 1994], where time is assumed to evolve linearly.  Transitions between states carry constraints on time and clocks may be reset if needed. This formalism is convenient to describe systems that show discrete and continuous behaviour.
%Specification of attack trees can be done by representing each node of the attack tree through a timed automaton, yielding a network of automata. 

% Priced Timed Automata
%Priced timed automata extend timed automata by allowing a specification of the cost accumulated during behaviour. This construction has been motivated by the application of timed automata to solve optimal scheduling and planning problems \cite{Behrmann2005}, but it can be applied in many other areas.
 
% UPPAAL Cora
%UPPAAL CORA is a model checking tool that allows Cost Optimal Reachability Analysis [Uppaal Cora, 2020] developed from researcher from Uppsala University and Aalborg University. It models real-time systems as a network of timed automata that carries some data (bounded integers or arrays). UPPAAL CORA then identifies optimal paths to a goal state under certain conditions, i.e., successful paths with minimal cost [Behrmann, 2001].
%The tools graphical user interface enables simple construction of the model to be investigated (see Figure 2 1 for a small example). Simulations of the designed model under certain restrictions, i.e., with time bounds, can be performed and return information on the model’s behaviour. 

==> preamble/authors.tex <==
\author{
    \IEEEauthorblockN{
        Thorsten Tarrach\IEEEauthorrefmark{1},
        Masoud Ebrahimi\IEEEauthorrefmark{2},
        Sandra König\IEEEauthorrefmark{1},
        Christoph Schmittner\IEEEauthorrefmark{1}, \\
        Roderick Bloem\IEEEauthorrefmark{2}, and
        Dejan Ničković\IEEEauthorrefmark{1}
    }
    \IEEEauthorblockA
    {
        \IEEEauthorrefmark{1}\, AIT Austrian Institute of Technology, Vienna, Austria
    }
    \IEEEauthorblockA
    {
        \IEEEauthorrefmark{2}\, Graz University of Technology, Graz, Austria
    }
    
}
